Resource Allocation for Downlink Channel Transmission Based on Superposition Coding

We analyze the problem of transmitting information to multiple users over a shared wireless channel. The problem of resource allocation (RA) for the users with the knowledge of their channel state information has been treated extensively in the literature where various approaches trading off the users' throughput and fairness were proposed. The emphasis was mostly on the time-sharing (TS) approach, where the resource allocated to the user is equivalent to its time share of the channel access. In this work, we propose to take advantage of the broadcast nature of the channel and we adopt superposition coding (SC)-known to outperform TS in multiple users broadcasting scenarios. In SC, users' messages are simultaneously transmitted by superposing their codewords with different power fractions under a total power constraint. The main challenge is to find a simple way to allocate these power fractions to all users taking into account the fairness/throughput tradeoff. We present an algorithm with this purpose and we apply it in the case of popular proportional fairness (PF). The obtained results using SC are illustrated with various numerical examples where, comparing to TS, a rate increase between 20% and 300% is observed.

==> Includes/Introduction.tex <==
\section{Introduction}\label{Sec:Introduction}
% what the paper is about
In this paper, we derive an \gls{ra} scheme for downlink multi-user communications where various utility functions may be applied. The distinctive feature of the analyzed scheme is that it is based on \gls{sc}. Unlike the popular and well studied \gls{ts} approach, where at each time instant only one user is receiving data, with \gls{sc} many users may receive their respective payload simultaneously.

% resource allocation : single user, 
In downlink communications over time-varying channels, \gls{ra} depends on the instantaneous channel condition between the \gls{bs} and the user (or \gls{ms}.) This usually results in transmission schemes which allocate resources (time, frequency, power) to the user which experiences the most favourable channel conditions.

% resource allocation : multiple users (multi-user diversity) 
In presence of multiple users, it was shown in \cite{Knopp95} that the optimal strategy to maximize the total throughput (sum-rate of all users) is to schedule the user with the best link during each transmission unit. This \gls{md} \cite[Ch.~6.6]{Tse05_Book} maximizes the overall system throughput by allocating the shared resource to the user that can best exploit it.
%
However, this approach raises a ``fairness'' issue since it would result in shared resources being monopolized by  the users with the best channel conditions (\eg with a direct link to the \gls{bs}, or at a short range from it), while the user with poor channel conditions would rarely access the channel affecting considerably his throughput. %

Total throughput enhancement and fairness are hence crucial but conflicting criteria in the design of optimal \gls{ra} schemes.

% the meaning of fairness and proportional fairness
To address this issue, many utility-based approaches---where utility represents a function of user's throughput---have been proposed in the literature to consider both fairness and throughput in the design of scheduling and \gls{ra} algorithms. Among them, \gls{pf} \cite{Kelly97}  based on the logarithmic utility function is a well-known criterion introduced to balance between throughput and fairness. Other approaches adopt different variants of the utility function but most of them can be reduced to the maximization of the weighted sum of users' throughputs. 

% time-sharing and superposition coding
Using \gls{pf} (or any other utility-based criterion) in the case of \gls{ts} leads to well-known and simple-to-implement results with the channel being allocated to a single user at any transmission time \cite{Kelly97,Berggren04}. On the other hand, it is also known that \gls{ts} approach is outperformed by \gls{sc} \cite[Ch.~15.1.3]{Cover06_Book} when communicating over shared (broadcast) channels. In \gls{sc}, the transmitter splits the available power among the multiple users, \emph{superimposes} the resulting codewords, and broadcasts them on the downlink channel. The underlying assumption is that the users are capable of decoding \gls{sc} signals via successive decoding. This is not a very restrictive assumption as the so-called hierarchical modulation, closely related to \gls{sc}, is nowadays included in communication standards, \eg \cite{Chari07}.

% the contribution of the paper
\gls{sc}-based \gls{ra} for cooperative communications was analyzed in \cite{Kaneko11,Thai13} but the formal analysis of multi-user \gls{sc} was not addressed therein. It was also studied in  \cite{Shaqfeh09,Zafar13}, where optimal solutions were derived using the approach of \cite{Tse97,Tse97b}. With respect to \cite{Shaqfeh09,Zafar13} our contributions are the following:
\begin{itemize}
\item We propose a very simple and optimal sorting-like algorithm, whose complexity is linear in the number of users. We derive it from the \gls{kkt} conditions applied directly to the \gls{ra} problem at hand. This is similar to the approach used by \cite{Zhang08} for the case of \gls{ts}. While the optimal results are the same as those that would result from an appropriate reorganization of the steps exposed in \cite{Shaqfeh09,Zafar13}, our approach does not require the formalism of \cite{Tse97,Tse97b}, it is hence simpler to derive and implement: the resulting algorithm can be straightforwardly used in presence of hundreds of scheduled users.
\item In the numerical examples we show that the gains provided by \gls{sc} combined with \gls{pf} criterion can lead to a multi-fold throughput increase for certain classes of users without penalty to the others. Moreover, we show that, in a single-cell scenario, the total throughput improves by up to 50\%  with respect to \gls{ts} with a growing number of users.
\item We observe that almost the entire power is distributed amongst just a few users. Motivated by this observation, we propose to apply \gls{sc} only to a limited number of users and propose the respective algorithms in this case.
\item We show that the two-user \gls{sc} is not only much more practical than the general multi-level superposition, but it also achieves most of the gains provided by unconstrained \gls{ra}. 
\end{itemize}

% organization of the paper
The rest of the paper is organized as follows. In \secref{Sec:Model}, we introduce the adopted transmission model, and in \secref{Sec:Sch.MD} we discuss \gls{ra} principles. We develop a simple algorithm to define the power allocation policy for \gls{sc} in \secref{Sec:PF.SC}, where we also analyze the case of power allocation under constraints on the number of scheduled users. % In \secref{Sec:Num.Results} we provide numerical examples that illustrate the advantages obtained thanks to the \gls{sc}-based transmission in  a simple case of scheduling in single-cell. 
Conclusions are drawn in \secref{Sec:Conclusions}.

==> Includes/Model.tex <==
\section{Transmission Model}\label{Sec:Model}
% independent block-fading channel model 
We consider the scenario where the \gls{bs} has to sent information to $L$ distinct users. We consider a frequency non-selective block-fading model commonly used in the analysis of wireless systems. Namely, we assume that at each time $n$, the signal received by the $l$-th user can be modelled as 
\begin{align}\label{}
y_{l}[n]=\sqrt{\SNR_{l}[n]}x[n]+z_{l}[n], \quad l=1,\ld, L,
\end{align}
where $x[n]$ is the unitary-power signal emitted by the \gls{bs}, $z_{l}[n]$ is the zero-mean  unitary variance random process modelling noise/interference, and $\SNR_{l}[n]$ is the \gls{snr} at the $l$-th receiver. 

In the block-fading model, for a given user $l$, the \gls{snr} is modelled as a white random process $\SNRrv_{l}[n]$. Thus, the \gls{snr}  stays constant for the duration of the entire block but varies independently between the blocks. 

While we do not assume any particular distribution to characterize the fading but, in the numerical examples we assume the Rayleigh fading, that is, the \gls{pdf} of  $\SNRrv$ is given by
\begin{align}\label{}
\pdf_{\SNRrv_{l}}(\SNR) = \frac{1}{\SNRav_{l}}\exp\left(-\frac{\SNR}{\SNRav_{l}}\right),
\end{align}
where $\SNRav$ is the average \gls{snr} of the $l$-th link.

We assume that at the beginning of each transmission block, each user informs \gls{bs} about the value of \gls{snr} $\SNR_{l}[n]$, which is possible thanks to the feedback channel.

Moreover, the \data to be sent to each of the users is available at the gls{bs} at any time instant $n$ (the so-called ``saturation'' case) and it is delay-insensitive, thus we can consider long-term averages as a relevant performance measures. These assumptions allow us to focus on the particular problem we want to address in this work, namely that of multi-user resource allocation considering \gls{sc}.

Knowing the \gls{snr} $\SNR_{l}[n]$, the central node must decide how to send the data to the receivers. This is known as \gls{ra}. In its most popular form, it boils down to the so-called ``scheduling'' which consists in dedicating entire block to a particular user indexed by $\ell[n]$, where the user's index allocation $\ell[n]$ depends on the scheduling strategy.

The transmission rate to the scheduled user $l=\ell[n]$, depends on the instantaneous \gls{snr} as 
 \begin{align}\label{rate.alloc.f}
r_{l}[n]=\phi(\SNR_{l}[n])
\end{align}
 The rate allocation function may take various forms, but here, for simplicity of analysis we use the capacity-achieving coding scheme
 \begin{align}\label{rate.alloc.Gauss}
\phi(\SNR)=\log(1+\SNR).
\end{align} 
That is, we consider the idealized case, where $x_{l}$ are obtained using infinite-length, randomly generated Gaussian codebook. In practice, of course, these assumptions cannot be met but allow us to focus on the allocation strategies and provide the upper limit on the rates achievable for any practical coding scheme. Despite this disclaimer, the rate allocation function we use may represent fairly well the performance of modern coding scheme based on strong, ``capacity-approaching'' codes, such as \glspl{tc} or \gls{ldpc} codes.

\subsection{Scheduling, Multi-User Diversity,  and Fairness}\label{Sec:Sch.MD}
% Round-Robin
The simplest scheduling is based on the so-called \gls{rr} approach where each user is assigned periodically (with period $L$) the entire transmission block, that is
\begin{align}\label{}
\ell[n]= n ~\mr{mod}~ L
\end{align}
where $\mr{mod}$ is the modulo operation.

Then each user utilizes exactly the same fraction $1/L$ of the overall transmission time and will receive data with an average rate
\begin{align}\label{}
R_{l}=\frac{1}{L}\Ex_{\SNRrv_{l}}[\phi(\SNRrv_{l})];
\end{align}
the same results in terms of the average rate will be obtained assigning each user a portion $\tau_{l}=1/L$ of the  block (if we ignore the practical limitation related to distributing the finite time $T$ among $L$ users).

The aggregate data rate is given by 
\begin{align}\label{}
R=\sum_{l=1}^{L}R_{l}.
\end{align}

Therefore, if all the users are in the same channel conditions, we have $R=\Ex_{\SNRrv_{l}}[\phi(\SNRrv_{l})]$. That is, increasing the number of users in the system the aggregate rate remains the same and each for them uses $1/L$ of it. This is because, while the information contained in the observations $\SNRvec[n]=[\SNR_{1}[n],\ld,\SNR_{L}[n]]$ is used to appropriately choose the transmission rate via rate-allocation function \eqref{rate.alloc.f}, the scheduling itself is independent of the the observed channel state $\SNRvec[n]$.
% Maximum rate allocation

If we are interested in increasing the aggregate rate we may consider the downlink transmission as a constant-power transmission to an ``aggregate'' user which combines all the users present in the system; then, irrespectively of the scheduling index $\ell[n]$ we are solely interested in the transmitted rate. Since the transmission is carried with constant power over parallel channels, it may be easily demonstrated that the maximum aggregate rate is obtained with the maximum-\gls{snr} scheduling
\begin{align}\label{max.G}
\ell[n]=\argmax_{l\in\set{1,\ld,L}}\SNR_{l}[n],
\end{align}
that is, we schedule for transmission the user with the largest instantaneous \gls{snr}. 

In such a case the  aggregate rate is larger than in the one obtained in \gls{rr} scheduling; in fact, the aggregate rate $R$ grows with the number of users. This effect is called \gls{md} to emphasize the fact that, thanks to the presence of many users whose \gls{snr} vary randomly, scheduling  increases the probability that the scheduled user experiences favourable conditions (high \gls{snr}).

While this strategy maximizes the aggregate rate $R$, there is a concern with respect to its ``fairness''. In the context of scheduling, the fairness is often defined with respect to the portions of time when the users are scheduled for transmission: if the fraction of the time the user was scheduled for transmission is comparable to $1/L$, we consider the scheduling to be fair. While \gls{rr} scheduling is fair by construction, using \eqref{max.G}, the user with the largest average \gls{snr} is scheduled more frequently than the user with weak \gls{snr}; this is often considered ``unfair''. 

It should be noted, however, that the fairness is not a well defined concept. For example, the fraction of the time when the user is  scheduled becomes less relevant if many users are simultaneously scheduled and transmit with different rate. In fact, in such a case, it is more convenient to talk about a more general concept of resource allocation which points out that various parameters of the transmission (resources) are allocated and not only the fraction of time (as it is the case when we consider the scheduling).

% Example comparing RR and MaxR

%The scheduling strategy $\mcS$ must at the same time provide large \gls{md} gains and guarantee fairness. It should  of course, be causal, \ie only the past channel realizations can be used to determine the scheduled user 
%\begin{align}\label{}
%\ell[n]=\mcS[\SNRvec[n-1], \SNRvec[n-2],\ld].
%\end{align}

\section{Proportionally fair ressource allocation}\label{Sec:PF}

To formalize the above considerations, we define the resource allocation policy $\mcS$ as a causal function of the channel states
\begin{align}\label{}
\bp[n]=\mcS\bigl(\SNRvec[n], \SNRvec[n-1], \ld, \SNRvec[n-W+1]\bigr)
\end{align}
where $\bp[n]\in\mcR$ is the set of parameters defining how the transmission to the users will be carried out, and the set of feasible solution $\mcR$ defines which parameters of the transmission can be modified, that is, what type of multi-user modulation/coding is allowed.

To ensure a fairness and take advantage of \gls{md}, various criteria have been proposed in the literature and the \gls{pf} resource allocation is among the most popular ones \cite{}. Its objective is to find the resource allocation policy  $\mcS^{\PF}(\cd)$ resulting in the the average rates $\hat{R}_{1}^\PF,\ld, \hat{R}_{L}^\PF $ such that for any other scheduling in the feasible parameters space $\mcR$, the sum of changes relative to $\hat{R}_{l}$ remains negative
\begin{align}\label{eq:PF.def}
   \sum_{l=1}^{L} \frac{R_{l}-\hat{R}_{l}^{\PF}}{R_{l}}\leq 0.
\end{align}

The advantage of \eqref{eq:PF.def} is that, it can be shown to be a solution of the following optimization problem
\begin{align}\label{sum.U}
\hat{\mcS}=\argmax_{\mcS} \sum_{l=1}^{L} U(R_{l}),
\end{align}
where $U(x)=\log(x)$ is the so-called utility function and the maximization is carried out over the possible policies $\mcS(\cd)$.
% Long-window approximation

To derive the optimal policy $\mcS$ we use  the time-average of the rate transmitted to the user,  using the length-$W$ window 
\begin{align}\label{R.n}
\tilde{R}_{l}[n]&=\frac{1}{W}\sum_{t=0}^{W-1}r_{l}[n-t]
=\frac{r_{l}[n]-r_{l}[n-W]}{W}+\tilde{R}_{l}[n-1],
\end{align}
where 
\begin{align}\label{r.t}
r_{l}[t]=\phi_{l}(\SNRvec[t],\bp[t])
\end{align}
is the rate conveyed to the $l$-th user at time $t$ and it depends on the channel state defined by the \glspl{snr} $\SNRvec[t]$ and the resource allocation $\bp[t]$, which is the outcome of the applied resource allocation policy $\mcS(\cd)$ at time $t$. The implicit in \eqref{r.t} is also the relationship to the multi-user modulation/coding.

The temporal averaging above is a convenient approximation particularly that, in order to calculate the true averages $R_{l}$ we would have to know the actual distribution of the \glspl{snr}. On the other hand, using time-averaged sequences, we let the resource allocation algorithms infer the actual channel statistics.

Using the time averages in \eqref{sum.U}, and assuming long observation windows, \ie $W\rightarrow\infty$, the optimization function may be approximated as
\begin{align}
\label{sum.U.n.1}
\hat{\bp}[n]&=\argmax_{\bp[n]}\sum_{l=1}^{L} \log\left(\tilde{R}_{l}[n-1]+\frac{r_{l}[n]}{W}\right)\\
\label{sum.U.n.2}
&=\argmax_{\bp[n]}\sum_{l=1}^{L} \log\left(1+\frac{r_{l}[n]}{\tilde{R}_{l}[n-1] W}\right) \\
\label{sum.U.n.3}
&=\argmax_{\bp[n]}\sum_{l=1}^{L} \frac{r_{l}[n]}{\tilde{R}_{l}[n-1]} \\
\label{sum.U.n.4}
&=\argmax_{\bp}\sum_{l=1}^{L} \frac{\phi_{l}(\SNRvec[n],\bp)}{\tilde{R}_{l}[n-1]} 
\end{align}
where, in \eqref{sum.U.n.1} we take advantage of the causality of the resource allocation policies, as well as we simplify \eqref{R.n}, neglecting the term $r_{l}[n-W]$ --justified, since for large $W$ we have $r_{l}[n-W]/W\ll\tilde{R}_{l}[n-1]$. In \eqref{sum.U.n.2} we remove the terms $\log(\tilde{R}[n-1])$ which, being independent of $\bp[n]$, do not affect the optimization, and in \eqref{sum.U.n.3} we use $\log(1+x)\approx x$ valid when $x\ll1$, which we are allowed to do because, as before, $r_{l}[n]/W\ll\tilde{R}_{l}[n-1]$ holds for large $W$. 

% TS PF

Considering the simple \gls{ts} multi-user modulation/coding scheme, which consists in assigning a fraction $p_{l}$ of the entire block to the $l$-th user, we have 
\begin{align}\label{phi.l.ts}
\phi_{l}^{\TS}(\SNRvec,\bp)=p_{l}\log(1+\SNR_{l})=p_{l}\phi(\SNR_{l})
\end{align}
and it is simple to see  that \eqref{sum.U.n.4}
\begin{align}\label{}
\hat{\bp}[n]=\argmax_{\bp}\sum_{l=1}^{L} \frac{p_{l}\phi(\SNR_{l}[n])}{\tilde{R}_{l}[n-1]},\quad \tnr{s.t.}\quad \sum_{l=1}^{L}p_{l}=1
\end{align}
is solved by scheduling for transmission only one user \cite[]{} indexed by
\begin{align}\label{eq:pf.ts}
\ell^{\PF}[n]=\argmax_{l\in\set{1,\ld, L}}\frac{\phi(\SNR_{l})}{\tilde{R}_{l}[n-1]},
\end{align}
that is, the optimal solution is given by $\hat{\bp}[n]=[0, 0 ,\ld, 1, \ld, 0 ]$ with a sole non-zero element at position $\ell^{\PF}[n]$.

This is the well-known \gls{pf-ts} resource allocation. The choice of the scheduled user depends on the ratio (proportion) between the instantaneous rate $\phi(\SNR_{l})$ and the rate that is allocated on the long run $\tilde{R}_{l}[n-1]\approx R_{l}$.  Thanks to the normalization by $R_{l}$, the users with relatively small average \gls{snr} (and thus also relative small value of $R_{l}$) are granted access to the channel more frequently than in the non-proportional max-\gls{snr} scheduling we outlined in \secref{Sec:Sch.MD}.

We note here that the maximization \eqref{sum.U} does not  optimize directly the criteria we are mostly interested in: the rates $R_{l}$. Moreover, the fairness, although present in the name of the optimization criterion, is not related to the concept we are most used to: fraction of the overall time used by the users. 

Nevertheless, despite the difficultly to relate the optimization to the ultimate objective of rate maximization and the constraints of fairness, the \gls{pf} criterion gained the popularity thanks to its simple formulation appearing in \eqref{sum.U.n.4}, particularly interesting as it yields easy to implement  \gls{pf-ts} scheduling policies given by  \eqref{eq:pf.ts}.

We will now take advantage of its simplicity in a slightly more involved multi-user modulation/coding scheme well adapted to the wireless downlink transmission.


==> Includes/Model_v2.tex <==
\section{Transmission Model}\label{Sec:Model}
% independent block-fading channel model 
We consider the scenario where the \gls{bs} has to sent information to $L$ distinct users. We consider a frequency non-selective block-fading model commonly used in the analysis of wireless systems. Namely, we assume that at each time $n$, the signal received by the $l$-th user can be modelled as 
\begin{align}\label{}
y_{l}[n]=\sqrt{\SNR_{l}[n]}x[n]+z_{l}[n], \quad l=1,\ld, L,
\end{align}
where $x[n]$ is the unitary-power signal emitted by the \gls{bs}, $z_{l}[n]$ is the zero-mean  unitary variance random process modelling noise/interference, and $\SNR_{l}[n]$ is the \gls{snr} at the $l$-th receiver. 

In the block-fading model, for a given user $l$, the \gls{snr} is modelled as a white random process $\SNRrv_{l}[n]$. Thus, the \gls{snr}  stays constant for the duration of the entire block but varies independently between the blocks. 

While we do not assume any particular distribution to characterize the fading but, in the numerical examples we assume the Rayleigh fading, that is, the \gls{pdf} of  $\SNRrv$ is given by
\begin{align}\label{}
\pdf_{\SNRrv_{l}}(\SNR) = \frac{1}{\SNRav_{l}}\exp\left(-\frac{\SNR}{\SNRav_{l}}\right),
\end{align}
where $\SNRav$ is the average \gls{snr} of the $l$-th link.

The data of each users is assumed available at the \gls{bs} at any time instant $n$ (the so-called ``saturation'' case) and it is delay-insensitive, thus we can consider long-term averages as a relevant performance measures.  Moreover, we assume that at the beginning of each transmission block, each user informs \gls{bs} about the value of \gls{snr} $\SNR_{l}[n]$, which is possible thanks to the feedback channel and we do not consider the related transmission overhead.

These assumptions allow us to focus on the particular problem we want to address in this work, namely that of multi-user resource allocation, in particular -- the one based on \gls{sc}.

The \gls{bs} at time $n$ forms the signal $x[n]$ using the \gls{mcs} $\phi(\cd)$ so that the rate conveyed to the user $l$ is given by
\begin{align}\label{}
r_{l}=\phi_{l}(\SNRvec[n],\bp[n]),
\end{align}
where $\bp[n]$ gathers all the parameters defining the \gls{mcs}. Choosing at each time $n$ the appropriate vector $\bp[n]$ is known as \gls{ra}. 

The simple and popular multi-user \gls{mcs} consists in \gls{ts}, where each user is assigned the fraction of the available transmission time so that
\begin{align}\label{phi.AWGN}
\phi_{l}^{\TS}(\SNRvec[n],\bp[n])=p_{l}[n]\log(1+\SNR_{l}[n]),
\end{align}
where, for simplicity of analysis we assume that \gls{mcs} uses the capacity-achieving coding. That is, we consider the idealized case, where $x_{l}$ are obtained using infinite-length, randomly generated Gaussian codebook. In practice, of course, these assumptions cannot be met but allow us to focus on the allocation strategies and provide the upper limit on the rates achievable for any practical coding scheme.\footnote{Despite this disclaimer, the rate function \eqref{phi.AWGN} represents well the performance of modern ``capacity-approaching'' codes, such as \glspl{tc} or \gls{ldpc} codes.}

\section{Scheduling, Multi-User Diversity,  and Fairness}\label{Sec:Sch.MD}
% Round-Robin
In the context of \gls{ts}, time is the resources to allocate to each user. Most often, the \gls{ra}  strategies consist in dedicating a transmission block to one particular user. This is called scheduling and the simplest one is based on the so-called \gls{rr} approach where each user is assigned periodically (with the period $L$) the entire transmission block. If we use $\boldsymbol{\delta}_{t}=[0, \ld, 0, 1, 0, \ld, 0]$ to denote the $L$-length vector with non-zero element at position $t$, then \gls{rr} can be described as
\begin{align}\label{}
\bp[n]&=\boldsymbol{\delta}_{t[n]}\\
t[n]&= [n-1]_{L} +1
\end{align}
where $[n]_{L}$ denotes  the modulo-$L$ operation.

Then, each user utilizes exactly the same fraction $1/L$ of the overall transmission time and will receive data with an average rate
\begin{align}\label{}
R_{l}=\frac{1}{L}\Ex_{\SNRrv_{l}}[ \log(1+\SNRrv_{l}) ];
\end{align}
the same results in terms of the average rate will be obtained assigning each user a portion $p_{l}=1/L$ of the  block (if we ignore the practical limitation related to distributing the finite time among $L$ users).

The aggregate data rate is given by 
\begin{align}\label{}
R=\sum_{l=1}^{L}R_{l}.
\end{align}

Therefore, if all the users are in the same channel conditions, we have $R=\Ex_{\SNRrv_{l}}[\phi(\SNRrv_{l})]$. That is, increasing the number of users in the system the aggregate rate remains the same and each user's average rate is $R/L$. In this case, the information contained in the observations $\SNRvec[n]$ is used to appropriately choose the transmission rate via rate-allocation function \eqref{phi.AWGN}, but the scheduling itself is independent of the the observed channel state $\SNRvec[n]$.

% Maximum rate allocation
If we are interested in increasing the aggregate rate we may consider the downlink transmission as a constant-power transmission to an ``aggregate'' user which combines all the users present in the system. As shown in \cite{} the maximum aggregate rate is obtained with the maximum-\gls{snr} scheduling
\begin{align}
\label{max.G.bp}
\bp[n]&=\boldsymbol{\delta}_{t[n]},\\
\label{max.G.tn}
t[n]&=\argmax_{l\in\set{1,\ld,L}}\SNR_{l}[n],
\end{align}
that is, we schedule for transmission the user with the largest instantaneous \gls{snr}. 

The  aggregate rate increases when comparing with \gls{rr} scheduling; and, it also grows with the number of users. This effect is called \gls{md} to emphasize the fact that, thanks to the presence of many users whose \gls{snr} vary randomly, scheduling  increases the probability that the scheduled user experiences favourable conditions (high \gls{snr}).

While this strategy maximizes the aggregate rate $R$, there is a concern with respect to its ``fairness''. In the context of scheduling, the fairness is often defined with respect to the portions of time when the users are scheduled for transmission: if the fraction of the time the user was scheduled for transmission is comparable to $1/L$, we consider the scheduling to be fair. While \gls{rr} scheduling is fair by construction, using \eqref{max.G}, the user with the largest average \gls{snr} is scheduled more frequently than the user with weak \gls{snr}; this is often considered ``unfair''. 

It should be noted, however, that the fairness is not a well defined concept. For example, the fraction of the time when the user is  scheduled becomes less relevant if many users are simultaneously scheduled and transmit with different rate. In fact, in such a case, it is more convenient to talk about a more general concept of resource allocation which points out that various parameters of the transmission (resources) are allocated and not only the fraction of time (as it is the case when we consider the scheduling).

% Example comparing RR and MaxR

%The scheduling strategy $\mcS$ must at the same time provide large \gls{md} gains and guarantee fairness. It should  of course, be causal, \ie only the past channel realizations can be used to determine the scheduled user 
%\begin{align}\label{}
%\ell[n]=\mcS[\SNRvec[n-1], \SNRvec[n-2],\ld].
%\end{align}

\section{Proportionally fair ressource allocation}\label{Sec:PF}

To formalize the above considerations, we define the resource allocation policy $\mcS$ as a causal function of the channel states
\begin{align}\label{}
\bp[n]=\mcS\bigl(\SNRvec[n], \SNRvec[n-1], \ld, \SNRvec[n-W+1]\bigr)
\end{align}
where $\bp[n]\in\mcR$ is the set of parameters defining how the transmission to the users will be carried out, and the set of feasible solution $\mcR$ defines which parameters of the transmission can be modified, that is, what type of multi-user modulation/coding is allowed.

To ensure a fairness and take advantage of \gls{md}, various criteria have been proposed in the literature and the \gls{pf} resource allocation is among the most popular ones \cite{}. Its objective is to find the resource allocation policy  $\mcS^{\PF}(\cd)$ resulting in the the average rates $\hat{R}_{1}^\PF,\ld, \hat{R}_{L}^\PF $ such that for any other scheduling in the feasible parameters space $\mcR$, the sum of changes relative to $\hat{R}_{l}$ remains negative
\begin{align}\label{eq:PF.def}
   \sum_{l=1}^{L} \frac{R_{l}-\hat{R}_{l}^{\PF}}{R_{l}}\leq 0.
\end{align}

The advantage of \eqref{eq:PF.def} is that, it can be shown to be a solution of the following optimization problem
\begin{align}\label{sum.U}
\hat{\mcS}=\argmax_{\mcS} \sum_{l=1}^{L} U(R_{l}),
\end{align}
where $U(x)=\log(x)$ is the so-called utility function and the maximization is carried out over the possible policies $\mcS(\cd)$.
% Long-window approximation

To derive the optimal policy $\mcS$ we use  the time-average of the rate transmitted to the user,  using the length-$W$ window 
\begin{align}\label{R.n}
\tilde{R}_{l}[n]&=\frac{1}{W}\sum_{t=0}^{W-1}r_{l}[n-t]
=\frac{r_{l}[n]-r_{l}[n-W]}{W}+\tilde{R}_{l}[n-1],
\end{align}
where 
\begin{align}\label{r.t}
r_{l}[t]=\phi_{l}(\SNRvec[t],\bp[t])
\end{align}
is the rate conveyed to the $l$-th user at time $t$ and it depends on the channel state defined by the \glspl{snr} $\SNRvec[t]$ and the resource allocation $\bp[t]$, which is the outcome of the applied resource allocation policy $\mcS(\cd)$ at time $t$. The implicit in \eqref{r.t} is also the relationship to the multi-user modulation/coding.

The temporal averaging above is a convenient approximation particularly that, in order to calculate the true averages $R_{l}$ we would have to know the actual distribution of the \glspl{snr}. On the other hand, using time-averaged sequences, we let the resource allocation algorithms infer the actual channel statistics.

Using the time averages in \eqref{sum.U}, and assuming long observation windows, \ie $W\rightarrow\infty$, the optimization function may be approximated as
\begin{align}
\label{sum.U.n.1}
\hat{\bp}[n]&=\argmax_{\bp[n]}\sum_{l=1}^{L} \log\left(\tilde{R}_{l}[n-1]+\frac{r_{l}[n]}{W}\right)\\
\label{sum.U.n.2}
&=\argmax_{\bp[n]}\sum_{l=1}^{L} \log\left(1+\frac{r_{l}[n]}{\tilde{R}_{l}[n-1] W}\right) \\
\label{sum.U.n.3}
&=\argmax_{\bp[n]}\sum_{l=1}^{L} \frac{r_{l}[n]}{\tilde{R}_{l}[n-1]} \\
\label{sum.U.n.4}
&=\argmax_{\bp}\sum_{l=1}^{L} \frac{\phi_{l}(\SNRvec[n],\bp)}{\tilde{R}_{l}[n-1]} 
\end{align}
where, in \eqref{sum.U.n.1} we take advantage of the causality of the resource allocation policies, as well as we simplify \eqref{R.n}, neglecting the term $r_{l}[n-W]$ --justified, since for large $W$ we have $r_{l}[n-W]/W\ll\tilde{R}_{l}[n-1]$. In \eqref{sum.U.n.2} we remove the terms $\log(\tilde{R}[n-1])$ which, being independent of $\bp[n]$, do not affect the optimization, and in \eqref{sum.U.n.3} we use $\log(1+x)\approx x$ valid when $x\ll1$, which we are allowed to do because, as before, $r_{l}[n]/W\ll\tilde{R}_{l}[n-1]$ holds for large $W$. 

% TS PF

Considering the simple \gls{ts} multi-user modulation/coding scheme, which consists in assigning a fraction $p_{l}$ of the entire block to the $l$-th user, we have 
\begin{align}\label{phi.l.ts}
\phi_{l}^{\TS}(\SNRvec,\bp)=p_{l}\log(1+\SNR_{l})=p_{l}\phi(\SNR_{l})
\end{align}
and it is simple to see  that \eqref{sum.U.n.4}
\begin{align}\label{}
\hat{\bp}[n]=\argmax_{\bp}\sum_{l=1}^{L} \frac{p_{l}\phi(\SNR_{l}[n])}{\tilde{R}_{l}[n-1]},\quad \tnr{s.t.}\quad \sum_{l=1}^{L}p_{l}=1
\end{align}
is solved by scheduling for transmission only one user \cite[]{} indexed by
\begin{align}\label{eq:pf.ts}
\ell^{\PF}[n]=\argmax_{l\in\set{1,\ld, L}}\frac{\phi(\SNR_{l})}{\tilde{R}_{l}[n-1]},
\end{align}
that is, the optimal solution is given by $\hat{\bp}[n]=[0, 0 ,\ld, 1, \ld, 0 ]$ with a sole non-zero element at position $\ell^{\PF}[n]$.

This is the well-known \gls{pf-ts} resource allocation. The choice of the scheduled user depends on the ratio (proportion) between the instantaneous rate $\phi(\SNR_{l})$ and the rate that is allocated on the long run $\tilde{R}_{l}[n-1]\approx R_{l}$.  Thanks to the normalization by $R_{l}$, the users with relatively small average \gls{snr} (and thus also relative small value of $R_{l}$) are granted access to the channel more frequently than in the non-proportional max-\gls{snr} scheduling we outlined in \secref{Sec:Sch.MD}.

We note here that the maximization \eqref{sum.U} does not  optimize directly the criteria we are mostly interested in: the rates $R_{l}$. Moreover, the fairness, although present in the name of the optimization criterion, is not related to the concept we are most used to: fraction of the overall time used by the users. 

Nevertheless, despite the difficultly to relate the optimization to the ultimate objective of rate maximization and the constraints of fairness, the \gls{pf} criterion gained the popularity thanks to its simple formulation appearing in \eqref{sum.U.n.4}, particularly interesting as it yields easy to implement  \gls{pf-ts} scheduling policies given by  \eqref{eq:pf.ts}.

We will now take advantage of its simplicity in a slightly more involved multi-user modulation/coding scheme well adapted to the wireless downlink transmission.


==> Includes/Model_v3.tex <==
\section{Transmission Model}\label{Sec:Model}
% independent block-fading channel model 
We consider the scenario where the \gls{bs} has to send information to $L$ distinct users. We consider a flat block-fading model commonly used in the analysis of wireless systems. Namely, we assume that at each time $n$, the signal received by the $l$-th user can be modeled as 
\begin{align}\label{}
y_{l}[n]=\sqrt{\SNR_{l}[n]}x[n]+z_{l}[n], \quad l=1,\ld, L,
\end{align}
where $x[n]$ is the unitary-power signal emitted by the \gls{bs}, $z_{l}[n]$ is the zero-mean  unitary variance random process modelling noise/interference, and $\SNR_{l}[n]$ is the \gls{snr} at the $l$-th receiver. 

In the block-fading model, for a given user $l$, the \gls{snr} is modelled as a white random process $\SNRrv_{l}[n]$. Thus, the \gls{snr}  stays constant for the duration of the entire block but varies independently between the blocks. 

While we do not need to assume any particular distribution to characterize the fading, we focus on the Rayleigh distribution in the numerical examples, that is, the \gls{pdf} of  $\SNRrv$ is given by
\begin{align}\label{}
\pdf_{\SNRrv_{l}}(\SNR) = \frac{1}{\SNRav_{l}}\exp\left(-\frac{\SNR}{\SNRav_{l}}\right),
\end{align}
where $\SNRav_{l}$ is the average \gls{snr} of the $l$-th link.

The data of each users is assumed available at the \gls{bs} at any time instant $n$ (the so-called ``saturation'' scenario) and it is delay-insensitive, thus we can consider long-term averages as a relevant performance measures.  Moreover, we assume that at the beginning of each transmission block, each user informs \gls{bs} about the value of \gls{snr} $\SNR_{l}[n]$, which is possible thanks to the feedback channel and we do not consider the related transmission overhead.

These assumptions allow us to focus on the particular problem we want to address in this work, namely that of multi-user resource allocation, in particular -- the one based on \gls{sc}.

The \gls{bs} at time $n$ forms the signal $x[n]$ using the \gls{mcs} $\phi(\cd)$ so that the rate conveyed to the user $l$ is given by
\begin{align}\label{}
r_{l}[n]=\phi_{l}(\SNRvec[n],\bp[n]),
\end{align}
where $\bp[n]$ gathers all the parameters defining the \gls{mcs}. Thus \gls{ra} consists in choosing at each time $n$ the appropriate vector $\bp[n]$. 

The simple and popular multi-user \gls{mcs} relies on time-sharing (\gls{ts}), where each user is assigned the fraction of the available transmission time so that
\begin{align}\label{phi.AWGN}
\phi_{l}^{\TS}(\SNRvec[n],\bp[n])=p_{l}[n]\log(1+\SNR_{l}[n]),
\end{align}
where, for simplicity of analysis, we assume that \gls{mcs} uses the capacity-achieving coding. That is, we consider the idealized case, where $x_{l}$ are obtained using infinite-length, randomly generated Gaussian codebook. In practice, of course, these assumptions cannot be met but allow us to focus on the allocation strategies and provide the upper limit on the rates achievable for any practical coding scheme.\footnote{Despite this disclaimer, the modern ``capacity-approaching'' codes, such as \glspl{tc} or \gls{ldpc} codes, when combined with appropriate modulation, yield rates well approximated by the  function \eqref{phi.AWGN}.}

% Round-Robin
In the context of \gls{ts}, time is the resource we have to allocate to each user.  Most often, the \gls{ra}  consists in dedicating the entire transmission block to one particular user. Then, the \emph{scheduling}, \ie determining which user transmits is equivalent to the \gls{ra}. The simplest \gls{ra} scheme is based on the so-called \gls{rr} approach where each user is assigned periodically (with the period $L$) the entire transmission block, thus
\begin{align}\label{}
\bp[n]&=\boldsymbol{\delta}_{t^{\tr{RR}}[n]}\\
t^{\tr{RR}}[n]&= \llbracket n-1\rrbracket _{L} +1
\end{align}
where we use $\boldsymbol{\delta}_{t}=[0, \ld, 0, 1, 0, \ld, 0]$ to denote the $L$-length vector with non-zero element at position $t$, and $\llbracket \cd\rrbracket _{L}$ denotes  the modulo-$L$ operation.

Then, each user utilizes exactly the same fraction $1/L$ of the overall transmission time and its throughput is given by 
\begin{align}\label{Ex.R.l}
R_{l}=\frac{1}{L}\Ex_{\SNRrv_{l}}[ \log(1+\SNRrv_{l}) ];
\end{align}
the same results in terms of the througput will be obtained assigning each user a portion $p_{l}=1/L$ of the  block (if we ignore the practical limitation related to distributing the finite time among $L$ users).

\section{Proportionally Fair Ressource Allocation}\label{Sec:Sch.MD}

The most often considered \gls{ra} strategies may be seen as the mapping $\mcS:\SNRvec\rightarrow\bp$ designed so as to maximize the sum of the so-called utility functions defined over the users' throughput $R_{l}$
\begin{align}\label{sum.U}
\hat{\mcS}=\argmax_{\mcS} \sum_{l=1}^{L} U(R_{l}),
\end{align}
where
\begin{align}\label{Ex.R.l}
R_{l}=\Ex_{\SNRrv_{1},\ld, \SNRrv_{L}}\left[\phi_{l}([\SNRrv_{1},\ld,\SNRrv_{L}],\bp)\right].
\end{align}

For example, using $U(R)=R$ corresponds to the maximization of the aggregate throughput $R=\sum_{l=1}^{L}R_{l}$ and it may be shown than in that case the optimal \gls{ra} is defined via \gls{ts} strategy, where only one user with the maximum instantaneous rate (MR) or \gls{snr} is scheduled for transmission within the block \cite{Berggren04}, \ie
\begin{align}
\label{max.SNR.1}
\bp[n]&=\boldsymbol{\delta}_{t^{\tr{MR}}[n]}\\
\label{max.SNR.2}
t^{\tr{MR}}[n]&=\argmax_{l\in\set{1,\ld,L}}\SNR_{l}[n].
\end{align}

However, \gls{ra} in \eqref{max.SNR.1}-\eqref{max.SNR.2} yields the results where the high-\gls{snr} users receive the highest throughput $R_{l}$, while weak-\gls{snr} users obtain small value of the $R_{l}$. This is considered ``unfair'' \cite{Berggren04}.

In order to  not penalize weak-\gls{snr} users various criteria have been proposed in the literature aiming to improve the fairness of the \gls{ra}. Among them,  the \gls{pf} criterion is arguably one of the most popular ones \cite{Kelly97}\cite{Zhang08} and corresponds to \eqref{sum.U} based on the utility function 
\begin{align}\label{Ux.log}
U(R)=\log(R).
\end{align}

\subsection{On-line adaptation}

Using $U(R)=R$, the mapping $\mcS$ is defined in closed-form via \eqref{max.SNR.1} and \eqref{max.SNR.2} but this is rarely the case. In fact, it is rather difficult to find the optimal mapping $\mcS$ for the popular utility function, such as the one in \eqref{Ux.log} corresponding to \gls{pf}. The main difficulty is to calculate in closed form the expectation \eqref{Ex.R.l}. 

In order to remedy this difficulty we may use the estimates of the throughput based on temporal averages\cite{Zhang08}
\begin{align}
\tilde{R}_{l}[n]&=\frac{1}{W}\sum_{t=0}^{W-1}r_{l}[n-t]\nonumber\\
\label{R.n}
&=\frac{r_{l}[n]-r_{l}[n-W]}{W}+\tilde{R}_{l}[n-1].
\end{align}

%The aggregate data rate given by 
%\begin{align}\label{}
%R=\sum_{l=1}^{L}R_{l}.
%\end{align}
%
%Therefore, if all the users are in the same channel conditions, we have $R=\Ex_{\SNRrv_{l}}[\phi(\SNRrv_{l})]$. That is, increasing the number of users in the system the aggregate rate remains the same and each user's average rate is $R/L$. In this case, the information contained in the observations $\SNRvec[n]$ is used to appropriately choose the transmission rate via rate-allocation function \eqref{phi.AWGN}, but the scheduling itself is independent of the the observed channel state $\SNRvec[n]$.

%It should be noted, however, that the fairness is not a well defined concept. For example, the fraction of the time when the user is  scheduled becomes less relevant if many users are simultaneously scheduled and transmit with different rate. In fact, in such a case, it is more convenient to talk about a more general concept of resource allocation which points out that various parameters of the transmission (resources) are allocated and not only the fraction of time (as it is the case when we consider the scheduling).

% Example comparing RR and MaxR

%The scheduling strategy $\mcS$ must at the same time provide large \gls{md} gains and guarantee fairness. It should  of course, be causal, \ie only the past channel realizations can be used to determine the scheduled user 
%\begin{align}\label{}
%\ell[n]=\mcS[\SNRvec[n-1], \SNRvec[n-2],\ld].
%\end{align}

Using \eqref{R.n} in \eqref{sum.U}, and assuming long observation windows, \ie $W\rightarrow\infty$, finding the optimal allocation parameters for the \gls{pf} utility function \eqref{Ux.log} may be formulated as the following optimization problem \cite{Zhang08}
\begin{align}
\label{sum.U.n.1}
\hat{\bp}^{\PF}[n]&=\argmax_{\bp[n]}\sum_{l=1}^{L} \log\left(\tilde{R}_{l}[n-1]+\frac{r_{l}[n]-r_{l}[n-W]}{W}\right)\\
%&\log\left(\tilde{R}_{l}[n-1]+\frac{r_{l}[n]-r_{l}[n-W]}{W}\right)\\
%&=\log\left(\tilde{R}_{l}[n-1](1+\frac{r_{l}[n]-r_{l}[n-W]}{W\tilde{R}_{l}[n-1]})\right)\\
%&=\log\left(\tilde{R}_{l}[n-1]\right)+\log\left(1+\frac{r_{l}[n]-r_{l}[n-W]}{W\tilde{R}_{l}[n-1]}\right)\\
\label{sum.U.n.3}
&\approx\argmax_{\bp[n]}\sum_{l=1}^{L}\frac{r_{l}[n]-r_{l}[n-W]}{\tilde{R}_{l}[n-1]}\\
%&=\log\left(\tilde{R}_{l}[n-1]\right)+1-\frac{r_{l}[n-W]}{W\tilde{R}_{l}[n-1]}+\frac{r_{l}[n]}{W\tilde{R}_{l}[n-1]}\\
%\label{sum.U.n.2}
%&=\argmax_{\bp[n]}\sum_{l=1}^{L} \log\left(1+\frac{r_{l}[n]}{\tilde{R}_{l}[n-1] W}\right) \\
%\label{sum.U.n.3}
%&=\argmax_{\bp[n]}\sum_{l=1}^{L} \frac{r_{l}[n]}{\tilde{R}_{l}[n-1]} \\
\label{sum.U.n.4}
&=\argmax_{\bp}\sum_{l=1}^{L} \frac{\phi_{l}(\SNRvec[n],\bp)}{\tilde{R}_{l}[n-1]}, 
\end{align}
The approximation sign in \eqref{sum.U.n.3} is due to application of the approximation $\log(1+x)\approx x$ valid when  $(r_{l}[n]-r_{l}[n-W])/W\ll\tilde{R}_{l}[n-1]$ -- the condition which holds for large $W$. The term $\frac{r_{l}[n-W]}{\tilde{R}_{l}[n-1]}$ is excluded from \eqref{sum.U.n.4} because it doesn't depend on $\bp$. 

We emphasize that the above adaptation rule is valid irrespectively of the \gls{mcs} we adopt, that is, may be applied for various forms of $\phi_{l}(\SNRvec,\bp)$.

\begin{example}[Proportional fairness in \gls{ts}]\label{ex:pf-ts}
Considering again \gls{ts}, we have to use \gls{mcs} where the rates are defined by \eqref{phi.AWGN}
and then \eqref{sum.U.n.4} becomes
\begin{align}\label{pf.ts.Opt}
\hat{\bp}^{\PF-\TS}[n]&=\argmax_{\bp}\sum_{l=1}^{L} \frac{p_{l}\log(1+\SNR_{l}[n])}{\tilde{R}_{l}[n-1]}\\
&\tnr{s.t.}\quad \sum_{l=1}^{L}p_{l}=1, p_{l}\geq 0.
\end{align}

It is easy to see that \eqref{pf.ts.Opt} is solved by scheduling for transmission only one user \cite{Zhang08} indexed by
\begin{align}\label{eq:pf.ts}
t^{\PF}[n]=\argmax_{l\in\set{1,\ld, L}}\frac{\log_{2}(1+\SNR_{l}[n])}{\tilde{R}_{l}[n-1]},
\end{align}
that is, the optimal solution is given by 
\begin{align}\label{eq:pf.bp}
\hat{\bp}^{\PF-\TS}[n]=\boldsymbol{\delta}_{t^{\PF}[n]}.
\end{align}
\end{example}

This is the well-known \gls{pf-ts} resource allocation. The choice of the scheduled user depends on the ratio (proportion) between the instantaneous achievable rate $\log(1+\SNR_{l}[n])$ and the throughput $\tilde{R}_{l}[n-1] \approx R_{l}$.  Thanks to the normalization by $R_{l}$, the users with relatively small average \gls{snr} (and thus also relative small value of $R_{l}$) are granted access to the channel more frequently than in the non-proportional max-\gls{snr} scheduling \eqref{max.SNR.1}-\eqref{max.SNR.2}.

We note that we do not  calculate explicitly the expectation \eqref{Ex.R.l}. Instead, by applying \eqref{eq:pf.ts} and \eqref{eq:pf.bp}, the \gls{ra} algorithm ``learns'' through the local optimization \eqref{pf.ts.Opt} what the globally optimal solution is.

Important common feature of all the mentioned \gls{ts} \gls{ra} schemes is that, in the $n$th block, only one user is scheduled for transmission. 

We will now take use \gls{pf} principle in a slightly more involved multi-user \gls{mcs} well suited for the wireless downlink transmission.


==> Includes/Model_v4.tex <==
\section{Transmission Model}\label{Sec:Model}
% independent block-fading channel model 
We consider the scenario where the \gls{bs} has to send information to $L$ distinct users. We consider the flat block-fading channel model commonly used in the analysis of wireless systems. Namely, we assume that at each discrete time instant $n$, the signal received by the $l$-th user is modeled as 
\begin{align}\label{}
y_{l}[n]=\sqrt{\SNR_{l}[n]}x[n]+z_{l}[n], \quad l=1,\ld, L,
\end{align}
where $x[n]$ is the unitary-power signal emitted by the \gls{bs}, $z_{l}[n]$ is the zero-mean  unitary variance random process modeling noise/interference, and $\SNR_{l}[n]$ is the \gls{snr} at the $l$-th receiver. 

In the block-fading model, for a given user $l$, the \gls{snr} is modelled as a white random process $\SNRrv_{l}[n]$. Thus, the \gls{snr} remains constant for the duration of the entire block but varies independently between blocks. 

While we do not need to assume any particular distribution to characterize the fading, we focus on the Rayleigh distribution in the numerical examples, that is, the \gls{pdf} of  $\SNRrv$ is given by
\begin{align}\label{}
\pdf_{\SNRrv_{l}}(\SNR) = \frac{1}{\SNRav_{l}}\exp\!\left(-\frac{\SNR}{\SNRav_{l}}\right),
\end{align}
where $\SNRav_{l}$ is the average \gls{snr} of the $l$-th link.

The data of each user is assumed available at the \gls{bs} at any time instant $n$ (the so-called ``saturation'' scenario) and it is delay-insensitive, thus we can consider long-term averages as relevant performance measures.  Moreover, we assume that at the beginning of each transmission block, each user informs the \gls{bs} about the value of its instantaneous \gls{snr} $\SNR_{l}[n]$, through a perfect feedback channel. We do not consider the related transmission overhead here it is out of the scope of the paper.
%which is possible thanks to the feedback channel and we do not consider the related transmission overhead.

These assumptions allow us to focus on the main problem addressed in this work; namely, multi-user resource allocation, and in particular -- the one based on \gls{sc}.

The \gls{bs} at time instant $n$ forms the signal $x[n]$ using the \gls{mcs} $\phi(\cd)$ so that the rate conveyed to the user $l$ is given by
\begin{align}\label{rl.def}
r_{l}[n]=\phi_{l}(\SNRvec[n],\bp[n]),
\end{align}
where $\bp[n]$ gathers all the parameters defining the \gls{mcs} and 
\begin{align}\label{snr.vec}
\SNRvec[n]=[\SNR_{1}[n],\ld,\SNR_{L}[n]].
\end{align}
%is the vector of values of each users's \gls{snr} at time $n$.

\gls{ra} consists, therefore, in choosing the appropriate vector $\bp[n]$. 

The simple and popular multi-user \gls{mcs} relies on time-sharing (\gls{ts}), where each user is assigned a fraction of the available transmission time so that
\begin{align}\label{phi.AWGN}
\phi_{l}^{\TS}(\SNRvec[n],\bp[n])=p_{l}[n]\log(1+\SNR_{l}[n]),
\end{align}
where, for simplicity, we assume that \gls{mcs} uses a capacity-achieving coding. That is, we consider the case, where signals $x_{l}$ are obtained from infinite-length, randomly generated Gaussian codebook. These idealistic assumptions allow us to focus on the allocation strategies and provide upper limits on the rates achievable for any practical coding scheme.%\footnote{Despite this disclaimer, the modern ``capacity-approaching'' codes, such as \glspl{tc} or \gls{ldpc} codes, when combined with appropriate modulation, yield rates well approximated by the  function \eqref{phi.AWGN}.}

% Round-Robin
In the context of \gls{ts}, \gls{ra} consists most often in dedicating the entire transmission time to one particular user. Then, \emph{scheduling} (\ie determining which user should transmit) is equivalent to a \gls{ra}. The simplest \gls{ra} scheme is based on the so-called \gls{rr} approach where each user is assigned periodically (with period $L$) to the entire transmission block, thus
\begin{align}\label{}
\bp[n]&=\boldsymbol{\delta}_{t^{\tr{RR}}[n]}\\
t^{\tr{RR}}[n]&= \llbracket n \rrbracket _{L} +1
\end{align}
where we use $\boldsymbol{\delta}_{t}=[0, \ld, 0, 1, 0, \ld, 0]$ to denote the $L$-length vector with a non-zero element at position $t$, and $\llbracket \cd\rrbracket _{L}$ denotes  the modulo-$L$ operation.

Then, each user occupies the channel during exactly the same fraction $1/L$ of the overall transmission time and its throughput is given by 
\begin{align}\label{RR.R.l}
R_{l}=\frac{1}{L}\Ex_{\SNRrv_{l}}[ \log(1+\SNRrv_{l}) ];
\end{align}
the same result in terms of throughput will be obtained assigning each user a portion $p_{l}=1/L$ of the  block (if we ignore the practical limitation related to distributing the finite time among $L$ users).

\section{Resource Allocation}\label{Sec:Sch.MD}

\gls{ra} strategies may be defined via a function $\bp=\bp(\SNRvec)$ designed to maximize the sum of the so-called utility functions defined over users' throughputs $R_{l}$
\begin{align}\label{sum.U}
\hat{\bp}(\SNRvec)=\argmax_{\bp(\SNRvec)} \sum_{l=1}^{L} U(R_{l}),
\end{align}
where
\begin{align}\label{Ex.R.l}
R_{l}=\Ex_{\SNRrvvec}\left[\phi_{l}\bigl(\SNRrvvec,\bp(\SNRrvvec)\bigr)\right]
\end{align}
and
\begin{align}\label{}
\SNRrvvec=[\SNRrv_{1},\ld,\SNRrv_{L}]
\end{align}
is the random vector modeling \eqref{snr.vec}.

For example, using $U(R)=R$ corresponds to the maximization of the aggregate throughput $R=\sum_{l=1}^{L}R_{l}$ and it can be shown then that the optimal \gls{ra} is defined via \gls{ts} with only one user (having the maximum instantaneous rate (MR) or --equivalently, the maximum \gls{snr}) is scheduled for transmission within the block \cite{Berggren04}, \ie
\begin{align}
\label{max.SNR.1}
\bp[n]&=\boldsymbol{\delta}_{t^{\tr{MR}}[n]}\\
\label{max.SNR.2}
t^{\tr{MR}}[n]&=\argmax_{l\in\set{1,\ld,L}}\SNR_{l}[n].
\end{align}

However, \gls{ra} in \eqref{max.SNR.1}-\eqref{max.SNR.2} results in a situation where the high-\gls{snr} users receive the highest throughput $R_{l}$, while weak-\gls{snr} users obtain lower throughputs $R_{l}$. This is considered ``unfair'' \cite{Berggren04}.

To avoid this, various criteria have been proposed in the literature aiming to improve the fairness of \gls{ra} algorithms. Among them,  the \gls{pf} criterion is arguably one of the most popular \cite{Kelly97}\cite{Zhang08} and corresponds to \eqref{sum.U} based on the utility function 
\begin{align}\label{Ux.log}
U(R)=\log(R).
\end{align}

On the other hand, the max-min optimization
\begin{align}\label{}
\hat{\bp}=\argmax_{\bp}\min_{l\in\set{1,\ld,L}}\set{R_{l}}
\end{align}
where resources are allocated so that the weakest user is prioritized, tend to yield \gls{er} \gls{ra}.

\subsection{On-line adaptation}

Using $U(R)=R$, the function $\bp(\SNRvec)$ is defined in closed-form via \eqref{max.SNR.1} and \eqref{max.SNR.2} but this is rarely the case. In fact, it is rather difficult to find the optimal mapping $\hat{\bp}(\SNRvec)$ for the popular utility function, such as the one in \eqref{Ux.log} corresponding to \gls{pf}. The main difficulty is to calculate the expectation \eqref{Ex.R.l} in closed form.

To overcome this problem, we may use estimates of the throughput based on temporal averages \cite{Zhang08}
\begin{align}
\tilde{R}_{l}[n]&=\frac{1}{W}\sum_{t=0}^{W-1}r_{l}[n-t]\nonumber\\
\label{R.n}
&=\frac{r_{l}[n]-r_{l}[n-W]}{W}+\tilde{R}_{l}[n-1].
\end{align}

Using \eqref{R.n} in \eqref{sum.U}, finding the optimal allocation parameters for the \gls{pf} utility function \eqref{Ux.log} can be formulated as the following optimization problem \cite{Zhang08}
\begin{align}
\label{sum.U.n.1}
\hat{\bp}[n]&=\argmax_{\bp[n]}\sum_{l=1}^{L} U\left(\tilde{R}_{l}[n-1]+\frac{r_{l}[n]-r_{l}[n-W]}{W}\right).
\end{align}
Further, for long observation windows, $W\rightarrow\infty$, \ie when 
\begin{align}\label{}
\frac{r_{l}[n]-r_{l}[n-W]}{W}\ll\tilde{R}_{l}[n-1],
\end{align}
we may use the first-order approximation $U(\tilde{R}+r)\approx U(\tilde{R})+U'(\tilde{R})\cd r$, which yields
%\begin{align}
%\label{sum.U.n.3}
%\hat{\bp}[n]&\approx\argmax_{\bp[n]}\sum_{l=1}^{L}U'(\tilde{R}_{l}[n])r_{l}[n]\\
%\label{sum.U.n.4}
%&\approx\argmax_{\bp[n]}\sum_{l=1}^{L}U'\bigl(\tilde{R}_{l}[n-1]\bigr) r_{l}[n]\\
%\label{sum.U.n.5}
%&\approx\argmax_{\bp[n]}\sum_{l=1}^{L}\beta_{l}[n] r_{l}[n]
%\end{align}
\begin{align}
\label{sum.U.n.3}
\hat{\bp}[n]&\approx\argmax_{\bp[n]}\sum_{l=1}^{L}U'\bigl(\tilde{R}_{l}[n-1]\bigr) r_{l}[n]\\
\label{sum.U.n.5}
&\approx\argmax_{\bp[n]}\sum_{l=1}^{L}\beta_{l}[n] r_{l}[n]
\end{align}
where the terms independent of $\bp$ (and hence not affecting the optimization results) were removed.% In \eqref{sum.U.n.4} we used $\tilde{R}_{l}[n]\approx\tilde{R}_{l}[n-1]$. 

The form of \eqref{sum.U.n.5}, emphasizes that the utility-function based approach may be reduced to the optimization of the sum of instantaneous rates $r_{l}[n]$ weighted by $\beta_{l}[n]=U'(\tilde{R}_{l}[n-1])$ \cite{Zafar13}. 

We emphasize that the adaptation rule \eqref{sum.U.n.5} is valid irrespectively of the adopted utility function or \gls{mcs}, that is, it may be applied for various forms of $\phi_{l}(\SNRvec,\bp)$ or $U(R)$. In particular, for $U(R)=R$ we recover the max-SNR (\ie also max-instantaneous rate $r_{l}[n]$) solution we have shown in \eqref{max.SNR.1}-\eqref{max.SNR.2}.

\begin{example}[Resource allocation in \gls{ts}]\label{ex:pf-ts}
Considering \gls{ts} again, we have to use \gls{mcs} with rates defined by \eqref{phi.AWGN}, thus
\eqref{sum.U.n.4} becomes
\begin{align}\label{pf.ts.Opt}
\hat{\bp}^{\PF-\TS}[n]&=\argmax_{\bp}\sum_{l=1}^{L} p_{l}\beta_{l}[n]\log_{2}(1+\SNR_{l}[n])\\
&\tnr{s.t.}\quad \sum_{l=1}^{L}p_{l}=1, p_{l}\geq 0.
\end{align}

It is easy to see that \eqref{pf.ts.Opt} is solved by scheduling only one user \cite{Zhang08} indexed by
\begin{align}\label{eq:pf.ts}
t[n]=\argmax_{l\in\set{1,\ld, L}}\beta_{l}[n]\log_{2}(1+\SNR_{l}[n]).
\end{align}

On the other hand, using the \gls{pf} utility function \eqref{Ux.log}, we obtain $U'(R)=R^{-1}$, thus $\beta_{l}[n]=1/\tilde{R}_{l}[n-1]$, \eqref{eq:pf.ts} becomes
\begin{align}\label{eq:pf.ts.2}
t^{\PF-\TS}[n]=\argmax_{l\in\set{1,\ld, L}}\frac{\log_{2}(1+\SNR_{l}[n])}{\tilde{R}_{l}[n-1]}.
\end{align}
and the optimal solution is given by 
\begin{align}\label{eq:pf.bp}
\hat{\bp}^{\PF-\TS}[n]=\boldsymbol{\delta}_{t^{\PF}[n]}.
\end{align}
\end{example}

This is the well-known \gls{pf-ts} resource allocation \cite{Liew08}. The choice of the scheduled user depends on the ratio (proportion) between the instantaneous achievable rate $\log(1+\SNR_{l}[n])$ and the throughput $\tilde{R}_{l}[n-1] \approx R_{l}$.  Thanks to the normalization by $R_{l}$, the users with relatively small average \gls{snr} (and thus also relative small value of $R_{l}$) are granted access to the channel more frequently than in the non-proportional max-\gls{snr} scheduling \eqref{max.SNR.1}-\eqref{max.SNR.2}.

We note that we do not  calculate explicitly the expectation \eqref{Ex.R.l}. Instead, by applying \eqref{eq:pf.ts} and \eqref{eq:pf.bp}, the \gls{ra} algorithm ``learns'' through the local optimization \eqref{pf.ts.Opt} what the globally optimal solution is.

An important common feature of all mentioned \gls{ra} schemes based on \gls{ts} is that, in the $n^\text{th}$ block, only one user is scheduled for transmission, that is \eqref{eq:pf.ts} is valid independently of the chosen utility-function. 


==> Includes/Numerical.tex <==
%\section{Numerical Example}\label{Sec:Num.Results}
\begin{example}[Downlink transmission to users in a cell]\label{ex:cell}
Let us compare now \gls{pf-sc},  \gls{pf-ts},  and \gls{rr} resource allocation strategies in a scenario which will highlight the most important properties of the proposed \gls{ra} beyond the simplified case of two groups of users we considered in \exref{ex:AB.users}.

%\subsection{Two groups of users}\label{Sec:L2.Numerical}
%\subsection{Users randomly distributed over a single-cell area}\label{Sec:Cell.Numerical}

Consider the case when $L$ users are distributed over a circular cell with a normalized radius $d_\tr{max}=1$. %The distance of the user $l$ to the \gls{bs} is denoted by $d_{l}$. 
We fix the \gls{snr} at the edge of the cell to $\SNRav(d_\tr{max})=0$dB and the average \gls{snr} at distance $d$ is given by $\SNRav(d)=d^{-\nu}$, where the path loss exponent is set to $\nu=3$ \cite{Liew08,Zafar13}. To avoid singularity (infinite \gls{snr}) at $d=0$, we set $\SNRav(d)=\SNRav(d_\tr{min})$ if $d\leq d_\tr{min}$ where $d_\tr{min}=0.1$, and the maximum \gls{snr} is thus $\SNRav(d_\tr{min})=30$dB.

We assume that the users are uniformly distributed over  the cell and since only their distance $d$ to the \gls{bs}  is important, we generate the latter as $d=\sqrt{x}$, where $x$ is uniformly distributed in $(0,1)$. Next, for all users at distance $d$, we calculate the average throughput, which we denote by $R(d)$. The positions of the users are randomly generated $N_\tr{rep}=1000$ times. In \figref{Fig:Rate.Dist}, we show the throughput as a function of the distance $R(d)$ for \gls{pf-ts}, \gls{pf-sc}, and \gls{rr} resource allocation strategies with $L=50$. 

These results are in line with the conclusions obtained from \exref{ex:AB.users}: the least populated groups of users (\ie those close to \gls{bs}) experience the greatest improvement in their throughput. For the case we analyze, when $d<0.35$ the increase is greater than 100\% and in the vicinity of the \gls{bs} we obtain a 300\% throughput gain.

At the same time, the throughput of all users is improved irrespectively of their distance $d$. This results in an increase of the aggregate throughput of the cell that we show in \figref{Fig:Rate.NUsers} as a function of the number of users $L$. We can appreciate that with respect to \gls{pf-ts}, the aggregate throughput of \gls{pf-sc} increases by 50\%  when $L>100$. 

As we have seen in \exref{ex:AB.users}, \gls{sc} tends to schedule more users with strong \gls{snr}, while keeping at least one weak-\gls{snr} user served. This explains the results of two-users \gls{sc} (denoted as $\SC_{2}$): the penalty due to  the constraint on the number of users $K_\tr{max}=2$ is more notable for strong-\gls{snr} users and is less important for users that are far from the \gls{bs}. Quite interestingly, there are no important differences between the throughput obtained via heuristic two-users \gls{ra} described in Algorithm~\ref{algo.greedy} and the optimal complex enumeration \eqref{Opt.SC.K}.

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\psfrag{distance}[ct][ct]{$d$}
\psfrag{ylabel}[c][c]{}%{$R(d)$}
\psfrag{SC-XXX-XXX-XXX-X}[cl][cl][0.9]{$R(d), \SC$}
\psfrag{SC-U2}[cl][cl][0.9]{$R(d), \SC_2, \tr{Opt.}$}
\psfrag{SC-U2-H}[cl][cl][0.9]{$R(d), \SC_{2}, \tr{Greedy}$}
\psfrag{TS}[cl][cl][0.9]{$R(d), \TS$}
\psfrag{RR}[cl][cl][0.9]{$R(d), \RR$}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/distance50.eps}}\
\caption{The throughput as a function of the normalized distance $d$ of the user from the \gls{bs};  $L=50$, the average \gls{snr} at the cell's edge is given by $\SNRav(1)=0$dB; $\SC_{2}$ refers to \gls{sc} under constraint $K_\tr{max}=2$, ``Opt.'' to the optimal exhaustive search \eqref{Opt.SC.K}, and ``Greedy'' to the results obtained via Algorithm~\ref{algo.greedy}.}\label{Fig:Rate.Dist}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\psfrag{xlabel}[ct][ct]{$L$}
\psfrag{ylabel}[c][c]{}%{$R(d)$}
\psfrag{SC-XXX-X}[cl][cl][0.9]{$R, \SC$}
\psfrag{TS}[cl][cl][0.9]{$R, \TS$}
\psfrag{RR}[cl][cl][0.9]{$R, \RR$}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/RatesD.eps}}\
\caption{The aggregate cell throughput as a function of the number of users $L$; the average \gls{snr} at the cell's edge is $\SNRav=0$dB.}\label{Fig:Rate.NUsers}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%
\end{example}


==> Includes/PF_SC.tex <==
\section{Resource allocation with superposition coding}\label{Sec:PF.SC}
%  Superposition Coding example 2 users
Before defining the framework for $L$ users it is convenient to analyze the case of $L=2$, which also clarifies the motivation for using \gls{sc}.

\subsection{Broadcasting  $L=2$}\label{Sec:2U.SC}
Consider the case of $L=2$ users with the \glspl{snr} $\SNR_{1}\leq \SNR_{2}$. From information-theoretic point of view, sending information to two users in the broadcast channel (\ie where both users receive each-other's signals) is done optimally via \gls{sc} \cite[Ch.~]{}. 

In the particular case of the Gaussian codebooks used by both users, and under mild conditions on the channel\footnote{The channel must be modelled as a physically degenerated broadcast channel \cite[]{}. This condition is satisfied in the case we treat here.}, the solution that maximizes the rate of the users $k=1$ and $k=2$ is obtained transmitting a superposition of  the codewords of both users, each of which, receives the signal
\begin{align}\label{}
y_{k}[n]=\sqrt{\SNR_{k}[n]}\left(\sqrt{p_{1}}x_{1}[n]+\sqrt{p_{2}}x_{2}[n]\right)+z_{k}[n],\quad k=1,2,
\end{align}
where $p_{k}$ are powers attributed to each user, and $p_{1}+p_{2}=1$ so that the  emitted signal $x[n]$ has unitary power.

The users then decode the signals they received: the stronger users should be able to decode all the messages, while the weak user should be able to decode only its own message. Since we assumed $\SNR_{1}\leq \SNR_{2}$, the user $k=1$ decodes only its own information treating the signal $x_{2}[n]$ as interference; the rate of reliable transmission is then given by
\begin{align}\label{rate.1.L2}
\phi_{1}^{\SC}(\bg,\bp)=\log_{2}\left(1+\frac{p_{1}\SNR_{1}}{p_{2}\SNR_{1}+1}\right),
\end{align}
where the denominator amalgams the power of the noise $z_{1}$ as well as the interference created by the signal  $\sqrt{p_{2}}x_{2}[n]$, which is possible because both are independent Gaussian variables. 

Since $\phi_{1}(\bg,\bp)$ is the increasing function of $\SNR_{1}$, the user $k=2$ (with $\SNR_{2}\geq \SNR_{1}$ ) can also play the role of the user $k=1$ and is able to decode the message $x_{1}$, remove it from the received signal, and the decoding is then based on the signal from which the interference has been canceled
\begin{align}\label{}
y'_{2}[n]=y_{2}[n]-\sqrt{\SNR_{2}[n]p_{1}}x_{1}=\sqrt{\SNR_{2}[n]p_{2}}x_{2}[n]+z_{2}[n]
\end{align}
so the resulting rate is 
\begin{align}\label{rate.2.L2}
\phi_{2}^{\SC}(\bg,\bp)=\log_{2}\left(1+p_{2}\SNR_{2}\right).
\end{align}

The parameters $\bp=[p_{1},p_{2}]$ determine the power allocated to the users and the level of interference user $k=1$ experiences due to the signal $x_{2}[n]$ of the user $k=2$. 

It is interesting to compare such a multi-user modulation/coding scheme with the \gls{ts} solution where the parameters $\bp$ play the role of the time-fraction of the time in the block and the achievable rates are given by \eqref{phi.l.ts}. This is done in \figref{} for two values of $\SNR_{1}=5$dB and $\SNR_{2}=10$dB. 

For \gls{ts} and \gls{sc} coding schemes, any pair of the transmission rates $\phi_{1}(\bg,\bp)$, $\phi_{2}(\bg,\bp)$ lying on the corresponding curve (or inside the region it delimits) can be obtained varying $p_{2}\in(0,1)$. Clearly any \gls{ts} solution is outperformed by \gls{sc} in terms of rates that be be transmitted to both users. Both schemes become equivalent for $p_{2}=0$ (only user $k=1$ transmits) or $p_{2}=1$ (only user $k=2$ transmits).

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\psfrag{xlabel}[c][c]{$\phi_{1}(\bg,\bp)$}
\psfrag{ylabel}[c][c]{$\phi_{2}(\bg,\bp)$}
\psfrag{XX1}{\gls{sc}}
\psfrag{X2}{\gls{ts}}
\psfrag{R1}[rc][rc]{$\phi(\SNR_{1})$}
\psfrag{Zx}[rc][rc]{$0$}
\psfrag{R2}[ct][ct]{$\phi(\SNR_{2})$}
\psfrag{R2b}[ct][ct]{$\phi(\SNR'_{2})$}
\psfrag{Zy}[ct][ct]{$0$}
\begin{center}
\scalebox{1}{\includegraphics[width=0.8\linewidth]{Figures/SCvsTS.eps}}
\caption{Rates $\phi_{1}(\bg,\bp)$ and $\phi_{2}(\bg,\bp)$ achievable with \gls{sc} and \gls{ts}; $\SNR'_{2}>\SNR_{2}$.}\label{Fig:SCvsTS}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
\subsection{Proportionally fair resource allocation for  $L=2$}\label{Sec:2U.SC}
Let us consider the case of the \gls{pf-sc} resource allocation for $L=2$. This will illustrate the main concept simplifying the solution for arbitrary $L$.

Using \eqref{rate.1.L2} and \eqref{rate.2.L2} in \eqref{sum.U.n.4} we have to solve the following maximization problem
\begin{align}\label{}
\hat{p}_{2}=\argmax_{p_{2}\in(0,1)}\log\frac{(1+p_{2}\SNR_{2})^{\tilde{R}_{1}}}{(1+p_{2}\SNR_{1})^{\tilde{R}_{2}}},
\end{align}
where, we explicitly took into account the constraint $p_{1}+p_{2}=1$ and--to alleviate the notation--we removed time indices, \ie $\SNR_{k}\equiv \SNR_{k}[n]$ and $\tilde{R}_{k}\equiv \tilde{R}_{k}[n-1]$.

After a simple algebra, the solution to this problem is given by:

\ls{AATA/REDOUANE: ici il faut expliquer la solution pour $L=2$}


For sufficiently large $W$, and when $n\rightarrow\infty$, the \gls{pf} resource allocation algorithm provides the optimal rates \cite{}, \ie $\tilde{R}_{k}[n] \rightarrow \hat{R}_{k}$. Then, the solution $\hat{\bp}$ depends solely on the values of the \glspl{snr}. 

It is instructive to compare the regions of \glspl{snr} $\bg=[\SNR_{1},\SNR_{2}]$ corresponding to different solutions in the case of \gls{pf-ts} and \gls{pf-sc}. This is shown in \figref{Fig:Regions.L2} assuming that $\hat{R}_{1}=1$ and $\hat{R}_{2}=2$ (these values do not correspond to any particular scenario) and are used for illustration purpose.

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\psfrag{xlabel}[c][c]{$\ov{SNR}$}
\psfrag{ylabel}[c][c]{BER}
\psfrag{XXXXXXX1}{$\alpha=1$}
\psfrag{XXXXX2}{$\hat{\alpha}$}
\psfrag{XXXXX3}{$\hat{\alpha}^\tr{GMI}$}
\psfrag{XXXXX4}{true L-values}
\psfrag{XXXXX5}{$\hat{\alpha}^{0}$}
\psfrag{TC}{TC}\psfrag{CC}{CC}
\begin{center}
%\scalebox{0.85}{\includegraphics[width=1.2\linewidth]{Figures/TS_SC_regions.eps}}
\caption{\ls{AATA: il faut montrer la figure de regions ici}.}\label{Fig:Regions.L2}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%
\subsection{Resource allocation for $L$ users}\label{Sec:SC.L}

The \gls{sc} transmission can be generalized to the case of $L$ users as follows: the transmitted signal is given by
\begin{align}\label{}
x[n]=\sum_{l=1}^{L}\sqrt{p_{l}}x_{l}[n]
\end{align}
where $\sum_{l=1}^{L}p_{1}=1$. Assuming $\SNR_{1}\leq \SNR_{2}\leq\ld\leq \SNR_{L}$, the decoding by the user $k$ is done similarly the case of $L=2$: the signals of weak users is decoded and subtracted in a successive-interference-cancellation manner we used before (only for the user $k=2$ when $L=2$), while the signal of strong users is treated as interference. The rate of reliable transmission to the user $k$ is then given by
\begin{align}\label{r.k.L}
\phi_{k}^{\SC}(\bg,\bp)=\log_{2}\left(1+\frac{p_{k}\SNR_{k}}{\ov{p}_{k}\SNR_{k}+1}\right),
\end{align}
where $\ov{p}_{k}=\sum_{l=k+1}^{K}p_{l}$ is the total power of users $k+1,k+2, \ld, L$.

\ls{ICI: on a besoin des explication de Redouane sur l'algorithme.}
To investigate the optimal solution $\hat{p}$ of the optimization problem \eqref{sum.U.n.4} we use what colled KKT conditions.\\
Let:
\begin{align}\label{}
y=\sum_{l=1}^{L} \frac{r_{l}[n]}{\tilde{R}_{l}[n-1]} 
\end{align}
$\hat{p}$ can be the optimal solution of \eqref{sum.U.n.4} only if there exists $\lambda$ satistfying :\\
\begin{align}\label{}
\frac{\partial y}{\partial p_{i}}(\hat{p_i})-\lambda\leq0,\\
(\hat{p_{i}})(\frac{\partial y}{\partial p_{i}}(\hat{p_i})-\lambda)=0
\end{align}
With this conditions we can conclude that :\\
\begin{align}\label{}
\frac{\partial y}{\partial p_{i}}(\hat{p_{i}})>\frac{\partial y}{\partial p_{i-1}}(\hat{p}_{i-1}) \Rightarrow \hat{p}_{i-1}=0,\\
\frac{\partial y}{\partial p_{i}}(\hat{p_{i}})<\frac{\partial y}{\partial p_{i-1}}(\hat{p}_{i-1}) \Rightarrow \hat{p_{i}}=0
\end{align}
Assuming $\SNR_{1}\leq \SNR_{2}\leq\ld\leq \SNR_{L}$ and after a simple derivation we get the following condition:\\
\begin{align}\label{}
\frac{\partial y}{\partial p_{i}}>\frac{\partial y}{\partial p_{i-1}} \Leftrightarrow \frac{snr_{i}\tilde{R}_{i-1}}{snr_{i-1}\tilde{R}_{i}}>\frac{1+\ov{p}_{i-1}snr_i}{1+\ov{p}_{i-1}snr_{i-1}}
\end{align}
\begin{definition}
let $p_{i,i-1}$ be the solution of the following equation:\\
\begin{align}\label{}
\frac{1+psnr_{i}}{1+psnr_{i-1}}=\frac{snr-{i}\tilde{R}_{i-1}}{snr-{i-1}\tilde{R}_{i}}
\end{align}
\end{definition}




==> Includes/PF_SC_v2.tex <==
\section{Optimal \gls{pf} with superposition coding}\label{Sec:PF.SC}
%  Superposition Coding example 2 users
Before defining the \gls{ra} framework based on the \gls{sc}, to clarify the motivation for using \gls{sc} we outline the principle of encoding/decoding for $L=2$.

\subsection{Broadcasting}\label{Sec:2U.SC}
From an information-theoretic point of view, sending information to the users over a shared channel (\ie where the users receive the same broadcasted signal) is done optimally via \gls{sc} \cite[Ch.~15.1.3]{Cover06_Book}. 

In the case of $L=2$ users, the solution that maximizes the sum of weighted rates of the users $l=1$ and $l=2$ is obtained transmitting a superposition of  the codewords, that is
\begin{align}\label{}
x[n]=\sqrt{p_{1}}x_{1}[n]+\sqrt{p_{2}}x_{2}[n]
\end{align}
where $p_{1}$ and $p_{2}$ are powers assigned to each of the users and $p_{1}+p_{2}=1$ so that the  emitted signal $x[n]$ has unitary power.

We assume without loss of generality that $\SNR_{1}\leq \SNR_{2}$ so the decoding  is done as follows : the weak-\gls{snr} user decodes only its own message $x_{1}[n]$ (treating the signal $x_{2}[n]$ as interference), and its achievable rate is then given by
\begin{align}\label{rate.1.L2}
\phi_{1}^{\SC}(\SNRvec,\bp)=\log_{2}\left(1+\frac{p_{1}\SNR_{1}}{p_{2}\SNR_{1}+1}\right),
\end{align}
where the denominator amalgams the power of the noise $z_{1}[n]$ as well as the interference created by the signal  $\sqrt{p_{2}}x_{2}[n]$, which is possible because both are independent Gaussian variables. 

Next, since $\phi_{1}^{\SC}(\SNRvec,\bp)$ is the increasing function of $\SNR_{1}$, the user $l=2$ (with $\SNR_{2}\geq \SNR_{1}$ ) can also decode the message $x_{1}[n]$ and remove it from the received signal $y_{2}[n]$ (we note that the message in $x_{1}[n]$ is discarded thus does not contribute to the throughput of the users $l=2$). The decoding of its own message $x_{2}[n]$ relies then on the signal from which the interference has been canceled
\begin{align}\label{}
y'_{2}[n]=y_{2}[n]-\sqrt{\SNR_{2}[n]p_{1}}x_{1}=\sqrt{\SNR_{2}[n]p_{2}}x_{2}[n]+z_{2}[n]
\end{align}
so the resulting rate is 
\begin{align}\label{rate.2.L2}
\phi_{2}^{\SC}(\SNRvec,\bp)=\log_{2}\left(1+p_{2}\SNR_{2}\right).
\end{align}

The parameters $\bp=[p_{1},p_{2}]$ determine the power allocated to the users and the level of interference user $l=1$ experiences due to the signal $x_{2}[n]$ of the user $l=2$. We emphasize here that the powers are allocated to both users using solely instantaneous values of \glspl{snr}. That is, we do not attempt to take advantage of the channel dynamics, done by the so-called \emph{water-filling} algorithms.

It is interesting to compare such a multi-user \gls{mcs} with the \gls{ts} solution where the parameters $\bp$ play the role of the time-fraction of the time in the block and the achievable rates are given by \eqref{phi.AWGN}. This is done in \figref{Fig:SCvsTS} for $\SNR_{1}<\SNR_{2}<\SNR'_{2}$. 

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\psfrag{xlabel}[c][c]{$\phi_{2}(\SNRvec,\bp)$}
\psfrag{ylabel}[c][c]{}%{$\phi_{1}(\SNRvec,\bp)$}
\psfrag{XX1-XXX}{$\phi_{1}^{\SC}(\SNRvec,\bp)$}
\psfrag{X2}{$\phi_{1}^{\TS}(\SNRvec,\bp)$}
\psfrag{p2=0}{$p_{2}=0$}
\psfrag{p2=1}{$p_{2}=1$}
\psfrag{R1}[rc][rc]{$\log(1+\SNR_{1})$}
\psfrag{Zx}[rc][rc]{$0$}
\psfrag{R2}[ct][ct]{$\log(1+\SNR_{2})$}
\psfrag{R2b}[ct][ct]{$\log(1+\SNR'_{2})$}
\psfrag{Zy}[ct][ct]{$0$}
\begin{center}
\scalebox{1}{\includegraphics[width=0.9\linewidth]{Figures/SCvsTS.eps}}
\caption{Rates $\phi_{1}(\SNRvec,\bp)$ vs. $\phi_{2}(\SNRvec,\bp)$ achievable with \gls{sc} and \gls{ts} and $\SNR_{1}<\SNR_{2}<\SNR'_{2}$. All the rates on the corresponding curves are achievable varying $p_{2}\in(0,1)$.}\label{Fig:SCvsTS}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%


Any pair of the transmission rates $\bigl(\phi_{1}(\SNRvec,\bp)$, $\phi_{2}(\SNRvec,\bp)\bigr)$  on the curve corresponding to \gls{ts} and \gls{sc}, can be obtained varying $p_{2}\in(0,1)$. Of course, the interpretation of the parameter $p_{2}$ depend on the \gls{mcs} we decide to use: for \gls{ts} $p_{2}$ has the meaning of the fraction of time, while for \gls{sc} it has the meaning of the fraction of the transmitted power. Clearly, for $0<p_{2}<1$ \gls{ts} solution is outperformed by \gls{sc} in terms of sum of rates to be transmitted to both users. The exception are  $p_{2}=0$ (only user $l=1$ transmits) or $p_{2}=1$ (only user $l=2$ transmits), when \gls{ts} and \gls{sc} are equivalent. 

We note also, that the advantage of using \gls{sc} instead of \gls{ts} becomes important when the difference between the \glspl{snr} of both users grows (note the difference between the \gls{sc} and \gls{ts} curves for $\SNR_{2}<\SNR'_{2}$). For $\SNR_{1}=\SNR_{2}$, \gls{ts} and \gls{sc} are equivalent.


The \gls{sc} transmission can be generalized to the case of $L>2$ as follows: the transmitted signal is given by
\begin{align}\label{}
x[n]=\sum_{l=1}^{L}\sqrt{p_{l}}x_{l}[n]
\end{align}
where $\sum_{l=1}^{L}p_{1}=1$. 

Assuming $\SNR_{1}\leq \SNR_{2}\leq\ld\leq \SNR_{L}$, the decoding by the user $l$ is done similarly the case of $L=2$: the signals of the weak users is decoded and subtracted in a successive-interference-cancellation manner we used before\footnote{When $L=2$, this is done only for $l=2$.}, while the signal of strong users is treated as the interference. Then, the rate of a reliable transmission to the user $l$ is given by
\begin{align}\label{r.k.L}
\phi_{l}^{\SC}(\SNRvec,\bp)=\log_{2}\left(1+\frac{p_{l}\SNR_{l}}{\ov{p}_{l}\SNR_{l}+1}\right),
\end{align}
where 
\begin{align}\label{ov.p}
\ov{p}_{l}=\sum_{j=l+1}^{L}p_{j}
\end{align} 
denotes the total power of users $l+1,l+2, \ld, L$, and $\ov{p}_{L}\triangleq 0$.

%%%%%%%%%%%%%%%%
\subsection{Resource allocation when $L=2$}\label{Sec:2U.SC}
For illustration purpose we consider now the case of the \gls{pf-sc} resource allocation for $L=2$.

If $\SNR_{1}<\SNR_{2}$, using \eqref{rate.1.L2} and \eqref{rate.2.L2} in \eqref{sum.U.n.5} we have to solve the following maximization problem
\begin{align}\label{p2.opt}
\hat{p}_{2}=\argmax_{p_{2}\in(0,1)}\log\frac{(1+p_{2}\SNR_{2})^{\tilde{R}_{1}}}{(1+p_{2}\SNR_{1})^{\tilde{R}_{2}}},
\end{align}
where, we explicitly took into account the constraint $p_{1}+p_{2}=1$ and--to alleviate the notation--we removed time indices, \ie $\SNR_{k}\equiv \SNR_{k}[n]$ and $\tilde{R}_{k}\equiv \tilde{R}_{k}[n-1]$.

Similarly, for $\SNR_{2}<\SNR_{1}$, we must solve
\begin{align}\label{p1.opt}
\hat{p}_{1}=\argmax_{p_{1}\in(0,1)}\log\frac{(1+p_{1}\SNR_{1})^{\tilde{R}_{2}}}{(1+p_{1}\SNR_{2})^{\tilde{R}_{1}}}.
\end{align}

After a simple algebra, the solution of \eqref{p2.opt} is given by:
\begin{enumerate}
\item if $\tilde{R}_{1} \ge \tilde{R}_{2}$ then $\hat{p}_{2}=1$
\item if $\tilde{R}_{1} < \tilde{R}_{2}$ we set :
\begin{align}
\label{alpha.12}
p_{2,1}=\frac{\tilde{R}_{1}\SNR_{2}-\tilde{R}_{2}\SNR_{1}}{\SNR_{1}\SNR_{2}(\tilde{R}_{2} -\tilde{R}_{1} )},
\end{align}
where the meaning of notation $p_{2,1}$ will become clear in the next section.
\begin{enumerate}
\item if $0\leq p_{2,1} \leq 1$ then $\hat{p}_{2}=p_{2,1}$
\item if $p_{2,1} \geq 1$ then $\hat{p}_{2}=1$
\item if $p_{2,1} \leq 0$ then $\hat{p}_{2}=0$.
\end{enumerate}
\end{enumerate}

It is interesting to compare the regions of \glspl{snr} $\SNRvec=[\SNR_{1},\SNR_{2}]$ corresponding to different solutions in the case of \gls{pf-ts} and \gls{pf-sc}. Assuming $n\rightarrow\infty$ (when the algorithms converges to the optimal solution), and for large $W$, using the \gls{pf} resource allocation algorithm we obtain $\tilde{R}_{k}[n] \rightarrow \hat{R}_{k}$ \cite{}. Therefore,  $\hat{R}_{k}$ are known and the solution $\hat{\bp}$ depends solely on the values of the \glspl{snr}. 

We shown in \figref{Fig:Regions.L2} the regions of $\SNRvec$ where different type of resource allocation are used.

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\psfrag{xlabel}[ct][ct]{$\SNR_{1}$}
\psfrag{ylabel}[cb][cb]{$\SNR_{2}$}
\psfrag{k}[ct][ct]{$\frac{\R_{2}}{R_{2}-R_{1}}$}
\psfrag{XXX}{$p_{2}^{\SC}=1$}
\psfrag{XXXX}{$p_{1}^{\SC}=1$}
\psfrag{XXXXX}{$p^{\TS}_{2}=1$}
\psfrag{XXXXXX}{$p^{\TS}_{1}=1$}
\psfrag{XXXXXXX}{$p^{ \SC}_{1}, p^{\SC}_{2}\in(0,1)$}
\begin{center}
\scalebox{1}{\includegraphics[width=0.9\linewidth]{Figures/TC_SC_regions.eps}}
\caption{Resource allocation regions in the domain of $\SNR_{1}$ and $\SNR_{2}$ for $L=2$ users when $\tilde{R}_{2}>\tilde{R}_{1}$. The decision regions for \gls{pf-ts} are shown hashed and those for \gls{pf-sc}-- shaded.}\label{Fig:Regions.L2}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%


%%%%
\subsection{Arbitrary number of users}\label{L.Users}

Defining the objective function in \eqref{sum.U.n.4} as
\begin{align}\label{y.SC}
y(\bp)=\sum_{l=1}^{L} \beta_{l}\phi^{\SC}_{l}(\SNRvec,\bp),
\end{align}
we have to solve now the following problem
\begin{align}\label{Opt.SC}
\hat{\bp}=\argmax_{\bp} y(\bp), \quad \tnr{s.t.}\quad \sum_{l=1}^{L}p_{l}=1, \quad p_{l }\geq 0.
\end{align}

This will be done in two optimal and interconnected steps
\begin{enumerate}
\item First, we find the indices $l$ of the users which must remain ``inactive'', that is, for which $\hat{p}_{l}=0$.
\item Next, for the remaining users, we obtain the optimal allocation of the power fractions $\hat{p}_{l}$.
\end{enumerate}

In the first step of the above approach, we use the \gls{kkt} conditions, as done also in\cite{Liew08}.%, which applied to \eqref{Opt.SC} yield the following relationship : %\cite{}, 
We know that there exists a Lagrange multiplier $\lambda$ such that the optimal solution of \eqref{Opt.SC} satisfies 
\begin{align}\label{}
\label{KKT.1}
\frac{\partial y(\hat{\bp}) }{\partial p_{l}}  -\lambda\leq0,\\
\label{KKT.2}
\hat{p}_{l}\left(\frac{\partial y(\hat{\bp})}{\partial p_{l}} -\lambda\right)=0,
\end{align}
The equality occurs in \eqref{KKT.1} only for $p_{l}>0$ so, for all $j,k\in\set{1,\ld, L}$, we can conclude with respect to the parameters $p_{l}$, for which the positivity constraints are active
\begin{align}\label{SC_KKT_1}
 \frac{\partial y(\hat{\bp})}{\partial p_{j}}>\frac{\partial y(\hat{\bp})}{\partial p_{k}} \Rightarrow \hat{p}_{k}=0,
%\frac{\partial y(\hat{\bp})}{\partial p_{l}} <\frac{\partial y(\hat{\bp})}{\partial p_{l-1}}  \Rightarrow \hat{p_{l}}=0
\end{align}
where, for brevity, we use $\frac{\partial y(\hat{\bp}) }{\partial p_{l}}\triangleq\frac{\partial y(\bp) }{\partial p_{l}} |_{\bp=\hat{\bp}}$. 

Assuming without loss of generality $j>k$, after simple algebra \ls{shown in Appendix}, \gls{lhs} of \eqref{SC_KKT_1} can be expressed as follows:
\begin{align}\label{SC_KKT_2}
\frac{\partial y(\hat{\bp})}{\partial p_{j}}>\frac{\partial y(\hat{\bp})}{\partial p_{k}} \Leftrightarrow \frac{\SNR_{j}\tilde{R}_{k}}{\SNR_{k}\tilde{R}_{j}}+\sum_{l=k+1}^{j-1}\hat{p}_{l}v_{l}>\frac{1+\hat{\ov{p}}_{k}\SNR_{j}}{1+\hat{\ov{p}}_{k}\SNR_{k}},
\end{align}
where $\sum_{l=k}^{k-1}a_{l}\triangleq 0$ takes care of the case $j=k+1$, and $v_{l}$ are arbitrary real numbers.

We will use now \eqref{SC_KKT_2} to identify the elements of $\hat{\bp}$, which must be equal to zero, \ie $\hat{p}_{l}=0$.

\begin{definition} 
Denote by $p_{j,k}$ the solution of 
\begin{align}
\label{f.p.jk}
\frac{1+p\SNR_{j}}{1+p\SNR_{k}}=\frac{\SNR_{j}\tilde{R}_{k}}{\SNR_{k}\tilde{R}_{j}}
\end{align}
with respect to $p$.
\end{definition}

%It is immediate to see that $p_{2,1}$ corresponds to $\alpha$ defined in \eqref{alpha.12}. 

\begin{proposition}\label{prop1}
If $j>k$ and $\sum_{l=k+1}^{j-1}\hat{p}_{l}=0$ then the following hold
\begin{align}
\label{Prop1.1}
\tilde{R}_{k}&\geq\tilde{R}_{j}&  &\Rightarrow &\hat{p}_{k}=0,\\
\label{Prop1.2}
\tilde{R}_{k}&<\tilde{R}_{j} \wedge p_{j,k}>1&  &\Rightarrow &\hat{p}_{k}=0,\\
\label{Prop1.3}
\tilde{R}_{k}&<\tilde{R}_{j} \wedge p_{j,k}<0&  &\Rightarrow &\hat{p}_{j}=0.
\end{align}
\begin{proof} In Appendix.
\end{proof}
\end{proposition}
\begin{proposition}\label{prop2}
If $m>j>k$, $\sum_{l=k+1}^{j-1}\hat{p}_{l}=0$, and $\sum_{l=j+1}^{m-1}\hat{p}_{l}=0$, then the following holds:
\begin{align}\label{prop2.1}
0&\leq p_{j,k}\leq p_{m,j}\leq 1 & & \Rightarrow & \hat{p}_{j}=0.
\end{align}
\begin{proof} In Appendix.
\end{proof}
\end{proposition}

Using \propref{prop1} and \propref{prop2} we may easily identify the terms $\hat{p}_{l}=0$. For convenience of considerations, we define the set $\mcL=\set{\ell_{1},\ld, \ell_{K}}$, which contains $K$ indices $\ell$, for which, the corresponding $\hat{p}_{\ell}$ are not zero.\footnote{Strictly speaking: those, for which we are not able to determine whether they are zero via \propref{prop1} and \propref{prop2}.} 

We can now define the ``expurgation'' algorithm, which verifies the conditions of \propref{prop1} and \propref{prop2}. We start assuming that the set contains all the indices, \ie $\mcL^{(0)}=\set{1,\ld, L}$, and  $K^{(0)}=L$; then we set $i=1$ and execute the following steps:
\begin{enumerate}
\item $\mcL^{(i)}\leftarrow \mcL^{(i-1)}$, 
\item $\forall l=1,\ld, K^{(i)}-1$, set $k=\ell_{l}, j=\ell_{l+1}$ and remove $\ell_{l}$ from $\mcL^{(i)}$ if \eqref{Prop1.1} or \eqref{Prop1.2} hold, and remove $\ell_{l+1}$ if \eqref{Prop1.3} holds.
\item $\forall l=2,\ld, K^{(i)}-1$, set $k=\ell_{l-1}, j=\ell_{l}, m=\ell_{l+1}$,  and remove $\ell_{l}$ from $\mcL^{(i)}$ if \eqref{prop2.1} holds.
\item $i\leftarrow i+1$.
\end{enumerate}
The above algorithm terminates when we cannot ``purge'' any more elements, thus when $\mcL^{(i)}=\mcL^{(i-1)}$.

We note that the decision whether $\hat{p}_{l}=0$ is made independently of the decision on $\hat{p}_{k}=0$, we can thus ``purge'' the inactive users (\ie those whose allocated powers are zero) using independent conditions. %Thus, even since we did not optimize the execution time, and theoretically it might take $L$ steps of the algorithm to stop, it usually requires a small number of iterations; we observed that it stops after \ls{REDOUANE: ici on a besoins d'un numero $i=XXXX$ steps.} 

\begin{example}[Finding the inactive users]
For the purpose of this example assume $L=5$, $\boldsymbol{\beta}=[]$ and $\SNRvec=[a,b,c,d,e]$.

We start calculating $p_{2,1}=$, $p{3,2}=$, $p_{5,4}=$.

\end{example}

The above algorithm produces the set $\mcL=\set{\ell_{1},\ell_{2},\ld,\ell_{K}}$ such that for any $l\in\mcL$,  $ p_{l}$ cannot be determined to be zero via \propref{prop1} or \propref{prop2}. Consequently, if $K=1$ there is only one non-zero power $p_{l}=1$, where $l=\ell_{1}$. Otherwise, all the elements of the set $\mcL$ satisfy the following condition
\begin{align}\label{ll.set}
0\leq p_{\ell_{K},\ell_{K-1}}<p_{\ell_{K-1},\ell_{K-2}}<\ld<p_{\ell_{2},\ell_{1}}\leq 1.
\end{align}

Then, to calculate the power fraction $p_{l}$ of the users indexed by $l\in\mcL$ we use:
\begin{proposition}\label{prop3} 
If $K>1$ and the elements of the set $\mcL$ satisfy \eqref{ll.set} then
\begin{align}
\label{prop3.1}
\hat{p}_{\ell_{K}}&=p_{\ell_{K},\ell_{K-1}}\\
\label{prop3.2}
\hat{p}_{\ell_{l}}&=p_{\ell_{l},\ell_{l-1}}-p_{\ell_{l+1},\ell_{l}}, \quad l=2,\ld, K-1, \\
\label{prop3.3}
\hat{p}_{\ell_{1}}&=1-p_{\ell_{2},\ell_{1}}
\end{align}	
\begin{proof} In Appendix.
\end{proof}		 
\end{proposition}


\subsection{\gls{ra} under constraints on the number of scheduled users}\label{}

Motivated by the results in \secref{Sec:Num.Results}, we analyze the \gls{ra} where we limit the number of users scheduled for transmission to $K_\tr{max}$
We will now analyze the case when we 

\subsection{Resource allocation under constraints on the users' power}\label{}


==> Includes/PF_SC_v3.tex <==
\section{Optimal \gls{ra} with superposition coding}\label{Sec:PF.SC}

We will now take the analysis of \gls{ra} based on utility-function to a more involved multi-user \gls{mcs} well suited for the wireless downlink transmission. While we use the \gls{pf} utility in the examples, \ie $\beta_{l}[n]=1/\tilde{R}_{l}[n-1]$, the presented solutions will be general, and remain valid when the utility function changes.

%  Superposition Coding example 2 users
To motivate the adoption of \gls{sc}, and before defining the \gls{ra} framework, we outline the principle of encoding/decoding based on \gls{sc}.

\subsection{\gls{sc} Broadcasting Principles}\label{Sec:2U.SC}
From an information-theoretic point of view, sending information to the users over a shared channel (\ie where the users receive the same broadcasted signal) is done optimally via \gls{sc} \cite[Ch.~15.1.3]{Cover06_Book}. 

In the case of $L=2$ users, the solution that maximizes the sum of weighted rates is obtained by transmitting a superposition of  the codewords, that is
\begin{align}\label{}
x[n]=\sqrt{p_{1}}x_{1}[n]+\sqrt{p_{2}}x_{2}[n]
\end{align}
where $x_{1}[n]$ and $x_{2}[n]$ are the unitary power signals of each user, $p_{1}$ and $p_{2}$ are their power fractions, and we impose the constraint $p_{1}+p_{2}=1$ so the  emitted signal $x[n]$ has a unitary power.

We assume without loss of generality that $\SNR_{1}\leq \SNR_{2}$. The decoding can be performaned as follows: the weak-\gls{snr} user decodes only its own message $x_{1}[n]$ (treating the signal $x_{2}[n]$ as interference). Since it receives the signal
\begin{align}\label{}
y_{1}[n]=\sqrt{\SNR_{1}p_{1}}x_{1}[n] + \sqrt{\SNR_{1}p_{2}}x_{2}[n] +z_{1}[n],
\end{align}
its achievable rate is given by
\begin{align}\label{rate.1.L2}
\phi_{1}^{\SC}(\SNRvec,\bp)=\log_{2}\left(1+\frac{p_{1}\SNR_{1}}{p_{2}\SNR_{1}+1}\right),
\end{align}
where the denominator of the fraction under the logarithm amalgams the power of the noise $z_{1}[n]$ as well as the interference created by the signal  $\sqrt{p_{2}}x_{2}[n]$, which is possible because both are independent Gaussian variables. 

User $l=2$ (with $\SNR_{2}\geq \SNR_{1}$) can also decode message $x_{1}[n]$ and remove it from the received signal 
\begin{align}\label{}
y_{2}[n]=\sqrt{\SNR_{2}}x[n]+z_{2}[n],
\end{align}
the decoding of his own message $x_{2}[n]$ relies then on the interference-free signal
\begin{align}\label{}
y'_{2}[n]=y_{2}[n]-\sqrt{\SNR_{2}[n]p_{1}}x_{1}[n]=\sqrt{\SNR_{2}[n]p_{2}}x_{2}[n]+z_{2}[n],
\end{align}
thus, the resulting rate is 
\begin{align}\label{rate.2.L2}
\phi_{2}^{\SC}(\SNRvec,\bp)=\log_{2}\left(1+p_{2}\SNR_{2}\right).
\end{align}

Since user $l=2$ discards the message contained in $x_{1}[n]$, decoding $x_{1}[n]$ does not contribute to his throughput.

Parameters $\bp=[p_{1},p_{2}]$ determine the power allocated to users and the level of interference user $l=1$ experiences due to the signal $x_{2}[n]$ of user $l=2$. We emphasize here that the powers are allocated to both users using solely instantaneous values of \glspl{snr}. That is, we do not attempt to take advantage of the channel dynamics, done by the so-called \emph{water-filling} algorithms.

To get an insight into the potential gains, \figref{Fig:SCvsTS} gives a comparison between \gls{sc} and \gls{ts}. %In the latter, the parameters $\bp$ play the role of the time-fraction of the time in the block and the achievable rates are given by \eqref{phi.AWGN}. This is done . 

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\newcommand{\scale}{0.8}
\psfrag{xlabel}[c][c]{$\phi_{2}(\SNRvec,\bp)$}
\psfrag{ylabel}[c][c]{}%{$\phi_{1}(\SNRvec,\bp)$}
\psfrag{XX1-XXX-X}[cl][cl][0.9]{$\phi_{1}^{\SC}(\SNRvec,\bp)$}
\psfrag{X2}[cl][cl][0.9]{$\phi_{1}^{\TS}(\SNRvec,\bp)$}
\psfrag{p2=0}[bl][bl][\scale]{$p_{2}=0$}
\psfrag{p2=1}[bl][bl][\scale]{$p_{2}=1$}
\psfrag{R1}[bc][cc][\scale][90]{$\log(1+\SNR_{1})$}
\psfrag{Zx}[rc][rc][\scale]{$0$}
\psfrag{R2}[ct][ct][\scale]{$\log(1+\SNR_{2})$}
\psfrag{R2b}[ct][ct][\scale]{$\log(1+\SNR'_{2})$}
\psfrag{Zy}[ct][ct][\scale]{$0$}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/SCvsTS.eps}}
\caption{Rates $\phi_{1}(\SNRvec,\bp)$ vs. $\phi_{2}(\SNRvec,\bp)$ achievable with \gls{sc} and \gls{ts} and $\SNR_{1}<\SNR_{2}<\SNR'_{2}$. Other rates on the corresponding curves are achievable varying $p_{2}\in(0,1)$.}\label{Fig:SCvsTS}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%


All pairs of transmission rates $\bigl(\phi_{1}(\SNRvec,\bp)$, $\phi_{2}(\SNRvec,\bp)\bigr)$  on the curves corresponding to \gls{ts} and \gls{sc}, can be obtained varying $p_{2}\in(0,1)$. Of course, the interpretation of the parameter $p_{2}$ depend on the \gls{mcs}: for \gls{ts} $p_{2}$ has a meaning of a time fraction, while for \gls{sc} it represents a fraction of the transmit power. Clearly, for any given rate $\phi_{1}(\SNRvec,\bp)$, using \gls{sc}, the rate of the remaining user $\phi_{2}(\SNRvec,\bp)$ can be always greater when comparing to the rate obtained via \gls{ts}. Exception are  $p_{2}=0$ (only user $l=1$ transmits) and $p_{2}=1$ (only user $l=2$ transmits), when \gls{ts} and \gls{sc} are equivalent. 

Moreover, we note that the advantage of using \gls{sc} instead of \gls{ts} becomes important when the difference between the \glspl{snr} of both users increases (note the difference between the \gls{sc} and \gls{ts} curves for $\SNR'_{2}>\SNR_{2}$); in fact, for $\SNR_{1}=\SNR_{2}$, \gls{ts} and \gls{sc} are equivalent.

\gls{sc} transmission can be generalized to the case of $L>2$ as follows: the transmitted signal is given by
\begin{align}\label{}
x[n]=\sum_{l=1}^{L}\sqrt{p_{l}}x_{l}[n]
\end{align}
where $\sum_{l=1}^{L}p_{l}=1$. 

Assuming $\SNR_{1}\leq \SNR_{2}\leq\ld\leq \SNR_{L}$, the decoding by the user $l$ is done similarly to the case of $L=2$: the signals of weak-SNR users are decoded and subtracted in a successive-interference-cancellation approach\footnote{When $L=2$, this is done only for $l=2$.}, while the signals of strong-SNR users are treated as interference. Then, the rate of a reliable transmission to user $l$ is given by
\begin{align}\label{r.k.L}
\phi_{l}^{\SC}(\SNRvec,\bp)=\log_{2}\left(1+\frac{p_{l}\SNR_{l}}{\ov{p}_{l}\SNR_{l}+1}\right),
\end{align}
where 
\begin{align}\label{ov.p}
\ov{p}_{l}=\sum_{j=l+1}^{L}p_{j}
\end{align} 
denotes the total power of users $l{+}1,l{+}2, \ld, L$. For convenience of notation, in what remains, we use
\begin{align}\label{sum.0}
\sum_{k=l}^{l-1}a_{k}\triangleq 0;
\end{align}
here, it means that $\ov{p}_{L}= 0$.

%%%%%%%%%%%%%%%%
\subsection{Resource allocation for $L=2$}\label{Sec:2U.SC.RA}
For illustration purposes, we now consider the case of \gls{ra} for $L=2$.

If $\SNR_{1}<\SNR_{2}$, using \eqref{rate.1.L2} and \eqref{rate.2.L2} in \eqref{sum.U.n.5} we have to solve the following maximization problem
\begin{align}\label{p2.opt}
\hat{p}_{2}=\argmax_{p_{2}\in(0,1)}\log\frac{(1+p_{2}\SNR_{2})^{\beta_{2}}}{(1+p_{2}\SNR_{1})^{\beta_{1}}},
\end{align}
where, the constraint $p_{1}+p_{2}=1$ is taken into account and---to alleviate the notation---we omit time indices, \ie $\SNR_{k}\equiv \SNR_{k}[n]$ and $\beta_{k}\equiv \beta_{k}[n]$.

Similarly, for $\SNR_{2}<\SNR_{1}$, we need to solve
\begin{align}\label{p1.opt}
\hat{p}_{1}=\argmax_{p_{1}\in(0,1)}\log\frac{(1+p_{1}\SNR_{1})^{\beta_{1}}}{(1+p_{1}\SNR_{2})^{\beta_{2}}}.
\end{align}

After a simple algebra, the solution of \eqref{p2.opt} is given by:
\begin{align}\label{p2.opt.L2}
\hat{p}_{2}=
\begin{cases}
1, & \!\!\!\tr{if~~}  \beta_{1}\!\le\!\beta_{2} \vee 
\displaystyle{\frac{\beta_{1}\SNR_{1}}{1+\SNR_{1}}\!\le\!\frac{\beta_{2}\SNR_{2}}{1+\SNR_{2}}}\\
0, & \!\!\!\tr{if~~}  \beta_{1}\SNR_{1}\!\ge\!\beta_{2}\SNR_{2}\\
\displaystyle{\frac{\beta_{2}\SNR_{2}-\beta_{1}\SNR_{1}}{\SNR_{1}\SNR_{2}(\beta_{1} -\beta_{2} )}},& \!\!\!\tr{otherwise}.
\end{cases}
\end{align}

%\begin{enumerate}
%\item if $\beta_{1} \le \beta_{2}$ then $\hat{p}_{2}=1$    
%\item if $\beta_{1} > \beta_{2}$ we set :
%\begin{align}
%\label{alpha.12}
%p_{2,1}=\frac{\beta_{2}\SNR_{2}-\beta_{1}\SNR_{1}}{\SNR_{1}\SNR_{2}(\beta_{1} -\beta_{2} )},
%\end{align}
%where the meaning of notation $p_{2,1}$ will become clear in the next section.
%\begin{enumerate}
%\item if $0\leq p_{2,1} \leq 1$ then $\hat{p}_{2}=p_{2,1}$
%\item if $p_{2,1} \geq 1$ then $\hat{p}_{2}=1$
%\item if $p_{2,1} \leq 0$ then $\hat{p}_{2}=0$.
%\end{enumerate}
%\end{enumerate}

Fixing $\boldsymbol{\beta}=[\beta_{1},\beta_{2}]$, the solution $\hat{\bp}$ depends solely on the values of the \glspl{snr}. In \figref{Fig:Regions.L2}, we illustrate how $\SNRvec$ affects the choice of $\hat{p}_{2}$ and compare \gls{sc} with \gls{ts}. Depending on the values of $\SNRvec$ and $\boldsymbol{\beta}$ we may obtain the solution equivalent to \gls{ts} (where we transmit to only one user) or to \gls{sc} where we transmit to both users simultaneously. 

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\newcommand{\scale}{0.8}
\psfrag{xlabel}[ct][ct]{$\SNR_{1}$}
\psfrag{ylabel}[cb][cb]{$\SNR_{2}$}
\psfrag{k}[ct][ct][\scale]{{\small$\displaystyle{\frac{\beta_{1}}{\beta_{1}{-}\beta_{2}}}$}}
\psfrag{XX-1}[cc][cc][\scale]{$p_{2}=1$}
\psfrag{XX-2}[cc][cc][\scale]{$\hat{p}_{2}=0$}
\psfrag{XX-3}[cc][cc][\scale]{$\hat{p}_{2}=p_{2,1}$}
\psfrag{XX-4}[cc][cc][\scale]{$\hat{p}_{2}=0$}
\psfrag{XX-1}[cc][cc][\scale]{$\hat{p}_{2}=1$}
\psfrag{TS-Limit}[tc][bc][\scale][57]{$\beta_{1}\log_{2}(1+\SNR_{1})=\beta_{2}\log_{2}(1+\SNR_{2})$}
\psfrag{SNR=Limit}[tc][bc][\scale][35]{$\SNR_{1}=\SNR_{2}$}
\psfrag{SNRbeta=Limit}[bc][tc][\scale][42]{$\SNR_{1}\beta_{1}=\SNR_{2}\beta_{2}$}
\psfrag{tau=Limit}[tc][bc][1][85]{$\frac{\beta_{1}\SNR_{1}}{1+\SNR_{1}} = \frac{\beta_{2}\SNR_{2}}{1+\SNR_{2}}$}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/TC_SC_regions.eps}}
\caption{Resource allocation may be seen as a mapping $\SNRvec\rightarrow\hat{\bp}$. Here, $L=2$ and  $\beta_{1}>\beta_{2}$ and \gls{ra} is defined via \eqref{p2.opt.L2}. The light-shaded regions correspond to the solution of the problem \eqref{p2.opt} (solved under assumption $\SNR_{2}>\SNR_{1}$) where only one user is scheduled for transmission ($\hat{p}_{1}=1$ or $\hat{p}_{2}=1$). The unshaded region corresponds to the case where we use \gls{sc}, \ie $\hat{p}_{1},\hat{p}_{2}\in(0,1)$. In the  dark-shaded region we have $\SNR_{2}<\SNR_{1}$ so the solution is found solving the problem \eqref{p1.opt}: through symmetry to the first case of \eqref{p2.opt.L2},  if $\SNR_{2}<\SNR_{1}$ and $\beta_{1}>\beta_{2}$ we set $\hat{p}_{1}=1$. The thick dashed (red) line separates the decision regions of \gls{ts}: above the line we schedule the user $l=2$ (thus $\hat{p}_{2}=1$), while below the line we schedule user $l=1$ ($\hat{p}_{1}=1$).}\label{Fig:Regions.L2}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%


%%%%
\subsection{Arbitrary number of users}\label{L.Users}

Our objective function in \eqref{sum.U.n.3} is now defined as 
\begin{align}\label{y.SC}
y_{\msL}(\bp)=\sum_{l=1}^{L} \beta_{l}\phi^{\SC}_{l}(\SNRvec,\bp).
\end{align}
where  we use $\msL=\set{1,2\ld, L}$ --the set integers from 1 to $L$, to emphasize that all the users are considered as the candidates for \gls{ra}; later, in \secref{sec:RA.Kmax}, we will consider the optimization under restrictions on the users that may be scheduled.

Then we have to solve the following optimization problem
\begin{align}\label{Opt.SC}
\hat{\bp}=\argmax_{\bp} y_{\msL}(\bp), \quad \tnr{s.t.}\quad \sum_{l=1}^{L}p_{l}=1, \quad p_{l }\geq 0.
\end{align}

This will be done in two optimal and interconnected steps:
\begin{enumerate}
\item First, we find indices $l$ of the users which are not scheduled for transmission, that is, for which $\hat{p}_{l}=0$.
\item Next, for the remaining users, we obtain the optimal allocation of power fractions $\hat{p}_{l}$.
\end{enumerate}

In the first step of the above approach, we use \gls{kkt} conditions, as done also in\cite{Liew08}. %, which applied to \eqref{Opt.SC} yield the following relationship : %\cite{}, 

We know that there exists a Lagrange multiplier $\lambda$ (associated with the constraint $\sum_{l=1}^{L}p_{l}=1$) and $\mu_{l}, l=1,\ld, L$ (each, associated with the constraint $p_{l}\geq 0$) such that the optimal solution of \eqref{Opt.SC} satisfies 
\begin{align}\label{}
\label{KKT.1}
\frac{\partial y_{\msL}(\hat{\bp}) }{\partial p_{l}}  -\lambda +\mu_{l}=0,
%\frac{\partial y(\hat{\bp}) }{\partial p_{l}}  -\lambda\leq0,\\
%\label{KKT.2}
%\hat{p}_{l}\left(\frac{\partial y(\hat{\bp})}{\partial p_{l}} -\lambda\right)=0
\end{align}
where $\mu_{l}\geq0$. If $\mu_{l}>0$ we say that the positivity constraint $p_{l}\geq 0 $ is active, and then $\hat{p}_{l}=0$. If $\mu_{l}=0$ the constraint is inactive.
%where inequality in \eqref{KKT.1} becomes equality if the positivity constraint $p_{l}\geq0$ is inactive.

We can then conclude with respect to the parameters $p_{l}$ for which the positivity constraints are active. Namely, for any $j,k\in\msL$ we have
\begin{align}\label{SC_KKT_1_1}
 \frac{\partial y_{\msL}(\hat{\bp})}{\partial p_{j}}>\frac{\partial y_{\msL}(\hat{\bp})}{\partial p_{k}} \Rightarrow \hat{p}_{k}=0,
%\frac{\partial y(\hat{\bp})}{\partial p_{l}} <\frac{\partial y(\hat{\bp})}{\partial p_{l-1}}  \Rightarrow \hat{p_{l}}=0
\end{align}
where, for brevity, we use $\displaystyle{\frac{\partial y_{\msL}(\hat{\bp}) }{\partial p_{l}}\triangleq\frac{\partial y_{\msL}(\bp) }{\partial p_{l}} |_{\bp=\hat{\bp}}}$.

Assuming without any loss of generality that $j>k$, and after simple algebra, the \gls{lhs} of \eqref{SC_KKT_1_1} can be expressed as follows:
\begin{align}\label{SC_KKT_2}
\frac{\partial y_{\msL}(\hat{\bp})}{\partial p_{j}}>\frac{\partial y_{\msL}(\hat{\bp})}{\partial p_{k}} \Leftrightarrow \frac{\SNR_{j}\beta_{j}}{\SNR_{k}\beta_{k}}+\sum_{l=k+1}^{j-1}\hat{p}_{l}v_{l}>\frac{1+\hat{\ov{p}}_{k}\SNR_{j}}{1+\hat{\ov{p}}_{k}\SNR_{k}},
\end{align}
where $\sum_{l=k}^{k-1}a_{l}\triangleq 0$ takes care of the case $j=k+1$, and $v_{l}$ are arbitrary real numbers.

We want to establish conditions under which the inequality \eqref{SC_KKT_2} is satisfied irrespectively of $\hat{\ov{p}}_{k}$, which will allow us to identify the elements of $\hat{\bp}$ to be made equal to zero, \ie $\hat{p}_{k}=0$ or $\hat{p}_{j}=0$.

\begin{proposition}\label{prop1}
If $j>k$ and $\sum_{l=k+1}^{j-1}\hat{p}_{l}=0$, then the following relationships hold:
\begin{align}
\label{Prop1.1}
\beta_{k}&\leq\beta_{j} \vee \tau_{k}<\tau_{j}&  &\Rightarrow &\hat{p}_{k}=0,\\
%\label{Prop1.2}
%\beta_{j}&<\beta_{k} \wedge \tau_{j}>\tau_{k}&  &\Rightarrow &\hat{p}_{k}=0,\\
\label{Prop1.3}
\beta_{k}&>\beta_{j} \wedge \nu_{k}>\nu_{j}&  &\Rightarrow &\hat{p}_{j}=0,
\end{align}
where
\begin{align}\label{}
\nu_{k}\triangleq\SNR_{k}\beta_{k},\\
\tau_{k}\triangleq\frac{\nu_{k}}{1+\SNR_{k}}
\end{align}
\begin{proof} \cf Appendix.
\end{proof}
\end{proposition}

\begin{definition}\label{def.1}
Denote by $p_{j,k}$ the solution of 
\begin{align}
\label{f.p.jk}
\frac{1+p\SNR_{j}}{1+p\SNR_{k}}=\frac{\nu_{j}}{\nu_{k}}
\end{align}
with respect to $p$.
\end{definition}

%It is immediate to see that $p_{2,1}$ corresponds to $\alpha$ defined in \eqref{alpha.12}. 

\begin{proposition}\label{prop2}
If $k<j<m$, $\sum_{l=k+1}^{j-1}\hat{p}_{l}=0$, and $\sum_{l=j+1}^{m-1}\hat{p}_{l}=0$, then the following holds:
\begin{align}\label{prop2.1}
0&\leq p_{j,k}\leq p_{m,j}\leq 1 & & \Rightarrow & \hat{p}_{j}=0.
\end{align}
\begin{proof} \cf Appendix.
\end{proof}
\end{proposition}

\propref{prop1} and \propref{prop2} allow us to ``purge'' users whose power fractions are zero $\hat{p}_{l}=0$. This can be done via simple element-by-element comparison between the parameters $\beta_{k}, \nu_{k}, \tau_{k}$, and $p_{j,k}$ using the algorithms we define below.  

To simplify the description of the algorithm, it is convenient to define a set $\mcL=\set{\ell_{1},\ell_{2},\ld,\ell_{K}}$ as the ordered set that gathers indices to $K$ ``non purged'' users, \ie for which we did not determine if $\hat{p}_{\ell_{k}}= 0 , k=1,\ld, K$. Then, purging user $l\in\mcL$ is equivalent to the elimination of his index $l$ from the set $\mcL$, which we denote as $\mcL\gets \mcL \backslash l$.

We start with Algorithm~\ref{Algo.1} which eliminates users according to \eqref{Prop1.1}. After this first purge, we use Algorithm~\ref{Algo.2} which enforces \eqref{Prop1.3}. Finally, we need to purge users using \propref{prop2} and, to this end, we proceed using  Algorithm~\ref{Algo.3}. 

%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[htb]
{\small
\caption{Purging users according to \eqref{Prop1.1}}	\label{Algo.1}
\begin{algorithmic}[1]
\REQUIRE $\beta_{l}, \tau_{l}$
\ENSURE Removes indices $l$ from the set $\mcL$ according to \eqref{Prop1.1}.
\STATE $\mcL \gets \msL$
\STATE $j\gets L$
\STATE $k\gets j-1$
\WHILE{$k\geq1$} 
	\IF{$\beta_{k}>\beta_{j} \wedge \tau_{k}>\tau_{j}$}
		\STATE $j \gets k$
	\ELSE
		\STATE $\mcL \gets \mcL \backslash k$
	\ENDIF
	\STATE $k\gets k-1$
\ENDWHILE
\end{algorithmic}
}
\end{algorithm}

%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[htb]
{\small
\caption{Purging users according to \eqref{Prop1.3}}	\label{Algo.2}
\begin{algorithmic}[1]
\REQUIRE $\nu_{l}, \mcL$
\ENSURE Removes indices $l$ from the set $\mcL$ according to \eqref{Prop1.3}.
\STATE $K \gets |\mcL|$
\STATE $k\gets 1$
\STATE $j\gets k+1$
\WHILE{$j\leq K$} 
	\IF{$\nu_{\ell_{k}}<\nu_{\ell_{j}}$}
		\STATE $k \gets j$
	\ELSE
		\STATE $\mcL \gets \mcL \backslash \ell_{j}$
	\ENDIF
	\STATE $j\gets j+1$
\ENDWHILE
\end{algorithmic}
}
\end{algorithm}


%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[htb]
{\small
\caption{Purging users according to \eqref{prop2.1} if $K>2$}	\label{Algo.3}
\begin{algorithmic}[1]
\REQUIRE $p_{k,j}, \mcL$
\ENSURE Removes indices $l$ from the set $\mcL$ according to \eqref{prop2.1}.
\STATE $K \gets |\mcL|$
\STATE $k\gets 1$
\STATE $j\gets k+1$
\STATE $m\gets k+2$
\WHILE{$m\leq K$} 
	\IF{$p_{\ell_{m},\ell_{j}}<p_{\ell_{j},\ell_{k}}$}
		\STATE $k \gets j$
	\ELSE
		\STATE $\mcL \gets \mcL \backslash \ell_{j}$
	\ENDIF
	\STATE $j \gets m$
	\STATE $m\gets m+1$
\ENDWHILE
\end{algorithmic}
}
\end{algorithm}

It is immediate to see that each of the above algorithms is executed using at most $L$ element-by-element comparisons. The total complexity is that linear in $L$.

Running Algorithm~\ref{Algo.3}, $K=|\mcL|$ users remain unpurged. We can now determine the optimal power-fractions.

If $K=1$, \ie there is only one user with non-zero power fraction, \ie $p_{\ell_{1}}=1$.

The following demonstrates that the conditions which allowed us to determine which users should have zero power-fractions are not only sufficient but also necessary.

\begin{proposition}\label{prop3} 
After applying Algorithm~\ref{Algo.1}, Algorithm~\ref{Algo.2}, and Algorithm~\ref{Algo.3}, the positivity constraints of all users remaining in the set $\mcL$ are inactive, \ie their Lagrange multipliers are $\mu_{\ell_{k}}=0, k=1,\ld, K$.
\begin{proof} \cf Appendix.
\end{proof}
\end{proposition}

Then, to find the power-fractions we can use the following.
\begin{proposition}\label{prop4}
If the number of users which are not purged via Algorithm~\ref{Algo.1}, Algorithm~\ref{Algo.2}, and Algorithm~\ref{Algo.3} is greater than one ($K>1$), the optimal solution of the problem in \eqref{Opt.SC} is found using the following rule:
\begin{align}
\label{prop3.1}
\hat{p}_{\ell_{K}}&=p_{\ell_{K},\ell_{K-1}}\\
\label{prop3.2}
\hat{p}_{\ell_{l}}&=p_{\ell_{l},\ell_{l-1}}-p_{\ell_{l+1},\ell_{l}}, \quad l=2,\ld, K-1, \\
\label{prop3.3}
\hat{p}_{\ell_{1}}&=1-p_{\ell_{2},\ell_{1}}
\end{align}	
\begin{proof} From \propref{prop3}, we know that $\mu_{\ell_{k}}=0$. Then, the optimality conditions in \eqref{KKT.1}, combined with \eqref{f.p.jk}, yield $p_{\ell_{j},\ell_{k}}=\hat{\ov{p}}_{\ell_{k}}$. This immediately yields the relationships in \eqref{prop3.1}, \eqref{prop3.2}, and \eqref{prop3.3}.
\end{proof}
\end{proposition}

\begin{example}[Optimal solution for $L=7$]

Suppose we have $L=7$ users with the following numerical values
\begin{align}\label{}
\SNRvec&=
[1.7,~ 3.3,~ 4.4,~ 6.7,~ 7.7,~ 8.3,~ 8.6]\\
\boldsymbol{\beta}&=
[6.0,~ 29.7,~ 26.5,~ 15.4,~ 4.6,~ 17.6,~ 12.2]
\end{align}


We are thus able to calculate
\begin{align}\label{}
\boldsymbol{\nu}&=[10.2, 98.0, 116.6, 103.2, 35.4, 146.1,104.9]\\
\boldsymbol{\tau}&=[~3.8,~ 22.8, ~21.6,~ ~13.4,~ 4.1,~ 15.7,~ ~10.9].
\end{align}

Running Algorithm~\ref{Algo.1}, we obtain
\begin{align}
\label{}
\SNRvec&=[\times, ~3.3, ~~~4.4, \times, ~\!\times, ~~8.3, ~~~8.6]\\
\label{nu.alog1}
\boldsymbol{\nu}&=[\times, 98.0, 116.6, \times, \times, 146.1, 104.9],
\end{align}
where we use ``$\times$'' to denote the irrelevant values corresponding to the purged users.

Using $\boldsymbol{\nu}$ from \eqref{nu.alog1} in Algorithm~\ref{Algo.2} we obtain
\begin{align}
\label{SNR.algo2}
\SNRvec&=[\times,~ 3.3, ~~4.4, \times, \times, ~8.3, \times]\\
\label{beta.algo2}
\boldsymbol{\beta}&=[\times, 29.7, 26.5, \times, \times, 17.6, \times].
\end{align}

The non-purged users are now indicated by the set \mbox{$\mcL=\set{2,3,6}$}, so we use \eqref{SNR.algo2} and \eqref{beta.algo2} in \eqref{f.p.jk} to calculate
\begin{align}\label{}
p_{6,3}=0.09, \qquad p_{3,2}=0.40,
\end{align}
and, after applying \propref{prop4}, we obtain the optimal solution
\begin{align}\label{}
\hat{p}_{6}&=0.09,\quad \hat{p}_{3}=0.31, \quad \hat{p}_{2}=0.60.
\end{align}

\end{example}

\begin{example}[Two groups of users and proportional fairness]\label{ex:AB.users}
We assume now that there are two groups of users, labeled ``A'' and ``B''. Each is composed, respectively, of $L_\tr{A}$ and $L_\tr{B}$ users having the same average \gls{snr}, $\SNRav_\tr{A}$ and $\SNRav_\tr{B}$, respectively. In \figref{Fig:Rate.A.B}, we show the throughput per user in each group: $R_\tr{A}$ and $R_\tr{B}$, for \gls{ra} strategies based on \gls{rr}, \gls{pf-ts}, and \gls{pf-sc}. 

We make the following observations:

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
\psfrag{SNR2(GB)}[ct][ct]{$\SNRav_\tnr{B}$}
\psfrag{ylabel}[c][c]{BER}
\psfrag{Throughput}{}
\psfrag{GB-SC-XX}{$R_\tr{B}$, \SC} \psfrag{GA-SC}{$R_\tr{A}$, \SC}
\psfrag{GB-TS}{$R_\tr{B}$, \TS} \psfrag{GA-TS}{$R_\tr{A}$, \TS}
\psfrag{GB-RR}{$R_\tr{B}$, \RR} \psfrag{GA-RR}{$R_\tr{A}$, \RR}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/Rate_AB_LA=4_LB=16_SNRA=0.eps}}\\
%\scalebox{1}{\includegraphics{Figures/Rate_AB_LA=4_LB=16_SNRA=0.eps}}\\
a)
\\
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/Rate_AB_LA=16_LB=4_SNRA=0.eps}}\\
%\scalebox{1}{\includegraphics{Figures/Rate_AB_LA=16_LB=4_SNRA=0.eps}}\\
b)
\caption{The throughput obtained using \gls{rr}, \gls{pf-ts}, and \gls{pf-sc} resource allocation policies for a)~$L_\tr{A}=4$, $L_\tr{B}=16$ and b)~$L_\tr{A}=16$, $L_\tr{B}=4$; $\SNRav_\tr{A}=0$dB.}\label{Fig:Rate.A.B}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%

\begin{enumerate}
\item The advantage of \gls{pf-sc} over \gls{pf-ts} is well pronounced when $\SNRav_\tr{A}$ and $\SNRav_\tr{B}$ differ significantly as then, \gls{sc} is most likely to provide notable gains. This is a reminiscence  of the broadcasting results for a fixed \gls{snr} shown in \secref{Sec:2U.SC}. 
\item Increasing the \gls{snr} of one group with respect to the other, the most significant throughput increase is obtained by the users in the least populated group irrespectively of their \gls{snr}:  their throughput grows by up to 100\% with respect to \gls{pf-ts}. For example, in \figref{Fig:Rate.A.B}a, we observe that increasing the \gls{snr} of group ``B'',  the throughput of users in group ``A'' improves by 100\%. This can be interpreted as follows: \gls{sc} tends to choose users with different \glspl{snr} as then the improvements over \gls{ts} are notable. Consequently, in the two-groups scenario, most likely one user from group ``A'' and one user from group ``B'' will be chosen. Thus, users in the least populated group are scheduled for transmission more frequently.
\item All users are drawing benefits from \gls{pf-sc} while this is not always the case for \gls{pf-ts}. In fact, the improvement in the throughput of group ``B'' is obtained by \gls{pf-ts} at the expense of the throughput of group ``A'' which decreases for large values of $\SNRav_\tr{B}$.
\end{enumerate}

Since in \gls{pf-sc} various users are simultaneously scheduled for transmission\footnote{We reuse the term ``scheduling'' to indicate that the power-fraction is not set to zero.} using \gls{sc}, it would be interesting to define how many can be simultaneously scheduled to allow the gains in \figref{Fig:Rate.A.B} to materialize. 

The number of users scheduled for transmission in groups ``A'' and ``B'' are denoted, respectively by $K_\tr{A}$ and $K_\tr{B}$. In \figref{Fig:Prob.A.B}, we show the empirical probability of the events corresponding to different pairs $(K_\tr{A}, K_\tr{B})$ that are the most likely to occur and we observe that
\begin{enumerate}
\item In most cases, the number of users scheduled for simultaneous transmission is relatively small: \mbox{$\Pr\set{K_\tr{A}+K_\tr{B}\leq3}>0.7$}. It is an important observation as \gls{sc} with a small number of users might be realized via practical \gls{mcs} such as the standard-defined hierarchical modulation \cite{Chari07}. 
\item The event $K_\tr{A}+K_\tr{B}=1$ means that only one user is scheduled, which is likely to happen for $\SNRav_\tr{B}\approx\SNRav_\tr{A}$, \ie where \gls{sc} and \gls{ts} are equivalent. The probability of using \gls{sc} increases when $\SNRav_\tr{B}$ increases, \ie when the difference between \glspl{snr} becomes significant. 
\item The most likely to be scheduled are users taken from group ``B'' ($K_\tr{B}=2$ or  $K_\tr{B}=3$) but even then, one of the users from group ``A'' is also scheduled. This explains the gains of \gls{pf-sc}: while we privilege high-\gls{snr} users from group ``B''; we still feed data to low-\gls{snr} users from group ``A'' using \gls{sc}. %This coincides with the proposition of \cite[Ch.~6]{Tse05_Book} who also suggests \gls{sc} scheme for downlink transmission transmitting to two users takes from different-\gls{snr} groups. We note, however, that we did not imposed such a condition and it is possible to activate users from the same group, \eg $\Pr\set{K_\tr{B}\geq2 \wedge K_\tr{A}=1}> 0.7$ for $\SNRav_\tr{B}=28$dB, \cf \figref{Fig:Prob.A.B}.
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\psfrag{SNR-B}[ct][ct]{$\SNRav_\tr{B}$}
\psfrag{Proba}[c][c]{}
\psfrag{P10-XXX-XXX-XXX}[cl][cl][0.9]{$K_\tr{A}+K_\tr{B}=1$}
\psfrag{P11}[cl][cl][0.9]{$K_\tr{A}=1, K_\tr{B}=1$}
\psfrag{P12}[cl][cl][0.9]{$K_\tr{A}=1, K_\tr{B}=2$}
\psfrag{P13}[cl][cl][0.9]{$K_\tr{A}=1, K_\tr{B}=3$}
\psfrag{P21}[cl][cl][0.9]{$K_\tr{A}=2, K_\tr{B}=1$}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/proba_AB_LA=4_LB=16_SNRA=0.eps}}\
a)\\
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/proba_AB_LA=16_LB=4_SNRA=0.eps}}\
b)
\caption{The height of the shaded area corresponds to the probability of simultaneous transmission to $K_\tr{A}$ users in group ``A'' and $K_\tr{B}$ users in group ``B'' for a)~$L_\tr{A}=4$, $L_\tr{B}=16$ and b)~$L_\tr{A}=16$, $L_\tr{B}=4$; $\SNRav_\tr{A}=0$.}\label{Fig:Prob.A.B}
%\caption{The height of the shaded area corresponds to the probability of simultaneous transmission to $K_\tr{A}$ users in the group ``A'' and $K_\tr{B}$ users in the group ``B'' when $L_\tr{A}=4$, $L_\tr{B}=16$, $\SNRav_\tr{A}=0$.}\label{Fig:Prob.A.B}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%

We not that the number of scheduled users does not convey the whole information as it does not reflect the values of the power-fractions $p_{l}$ which, indeed, can be very  small. In particular, let us define
\begin{align}\label{}
P_{2}=\max_{j,k\in\mcL}\set{p_{j}+p_{k}}.
\end{align}
as the maximum power attributed to two users. We show in \figref{Fig:Prob.alpha.A.B} the empirical probability
$\Pr\set{ P_{2}\in \mcP}$, where $\mcP$ is the interval of power values. We can observe that, even if the probability of having more that two users scheduled for transmission in the scenario  $L_\tr{A}=4$, $L_\tr{B}=16$ is relatively large (\figref{Fig:Prob.A.B}a), the power assigned to additional users (beyond the first two users) is small. In fact, in 90\% of the analyzed cases, the first two users obtain more than 80\% of the power. We do not show the case  $L_\tr{A}=16$, $L_\tr{B}=4$ for which $\Pr\set{ P_{2}\in (0.9,1]}>0.95$, \ie almost all the available power is assigned to the first two users.

%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\psfrag{SNR-B}[ct][ct]{$\SNRav_\tr{B}$}
\psfrag{Proba}[c][c]{}
\psfrag{P0-70-XXX-XXX-X}[cl][cl][0.9]{$\mcP=[0, 0.70)$}
\psfrag{P70-80}[cl][cl][0.9]{$\mcP=[0.70, 0.80)$}
\psfrag{P80-90}[cl][cl][0.9]{$\mcP=[0.80, 0.90)$}
\psfrag{P90-95}[cl][cl][0.9]{$\mcP=[0.90, 0.95)$}
\psfrag{P95-100}[cl][cl][0.9]{$\mcP=[0.95,1.0]$}
\begin{center}
\scalebox{1}{\includegraphics[width=1\linewidth]{Figures/proba_alpha_LA=4_LB=16.eps}}
\caption{The height of the shaded area corresponds to the probability that the power of the two strongest users $P_{2}$ belongs to the inteval $\mcP$; $L_\tr{A}=4$ $L_\tr{B}=16$, and $\SNRav_\tr{A}=0$.}\label{Fig:Prob.alpha.A.B}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%

\end{example}



\subsection{\gls{ra} under constraints on the number of scheduled users}\label{sec:RA.Kmax}

The numerical results in \exref{ex:AB.users} indicate that, with the optimal \gls{ra}, not only the number of users scheduled for transmission is small; but also the power of the first two users is dominant. This is interesting as, in practice, the number of superposed signals should not be very large. Thus, motivated by these results, we would like to obtain the \gls{ra} algorithm where we limit the number of users scheduled for transmission to a small value $K_\tr{max}$, and next, we will evaluate the penalty introduced by this additional constraint.

Our objective thus is to find the optimum indices $\hat{\mcL}=\set{\hat{\ell}_{1},\hat{\ell}_{2},\ld, \hat{\ell}_{K_\tr{max}}}$
\begin{align}\label{Opt.SC.K}
\hat{\mcL}&=\argmax_{\mcL\in \msL^{K_\tr{max}}} y_{\mcL}(\hat{\bp}_{\mcL}),
\end{align}
where
\begin{align}
\label{y.mcL.K}
y_{\mcL}(\hat{\bp}_{\mcL})&=\sum_{k=1}^{|\mcL|}\phi_{\ell_{k}}(\SNRvec,\hat{\bp}_{\mcL}),
\end{align}
and
\begin{align}
\label{Opt.SC.b.K}
\hat{\bp}_{\mcL}&=\argmax_{\bp} y_{\mcL}(\bp), \\ 
\nonumber
&\tnr{s.t.}\quad \sum_{k=1}^{|\mcL|}p_{\ell_{k}}=1, \quad p_{\ell_{k} }\geq 0 \\
\nonumber
&\qquad p_{l}=0\quad \tr{if}\quad l\notin\mcL
\end{align}
with $\msL^{K}$ being a $K$-fold Cartesian product of $\msL$.

This problem is more difficult than the optimization without constraint on the maximum number of allowed users $K_\tr{max}$. While the solution of \eqref{Opt.SC.b.K} has a linear complexity with $|\mc{L}|$, we have to repeat it for all the elements of the set $\msL^{K_\tr{max}}$; the overall complexity is then proportional to $L^{K_\tr{max}}$.

To avoid the polynomial complexity, we propose the greedy optimization algorithm described in Algorithm~\ref{algo.greedy}: starting with the empty set $\mcL=\emptyset$ we add one user at a time to maximize the overall objective function. While suboptimal, this algorithm provides a better solution than the \gls{ts}-based \gls{ra}. This is because the first user which is added to the set $\mcL$ is the one we find in the \gls{ts} approach, \cf \eqref{eq:pf.ts}. Other users are added to the set $\mcL$ solely if their presence improves the cost function. If this is not possible, and  the objective function does not increase (\ie the power-fraction attributed to the optimal user found in step \ref{step.opt} is zero $\hat{p}_{\hat{l}}=0$) the algorithm stops.

%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[htb]
{\small
\caption{Greedy maximization of the objective function: indices of active users are added to the set $\mcL$ one-by-one.}	\label{algo.greedy}
\begin{algorithmic}[1]
\REQUIRE $K_\tr{max}$
\ENSURE Suboptimal solution of the problem in \eqref{Opt.SC.K}.
\STATE $\mcL \gets \emptyset$
\STATE $K\gets 0$
\WHILE{$K\leq K_\tr{max}$} 
	\STATE $\hat{l}\gets \argmax_{l\in \msL, l \notin  \mcL} y_{\set{\mcL,l}}(\hat{\bp}_{\set{\mcL,l}})$\label{step.opt}
	\IF{$y_{\set{\mcL,\hat{l}}}\bigl(\hat{\bp}_{\set{\mcL,\hat{l}}}\bigr)>y_{\mcL}\bigl(\hat{\bp}_{\mcL}\bigr)$}
		\STATE $\mcL\gets \set{\mcL,\hat{l}}$
		\STATE $K\gets K+1$
	\ELSE
		\STATE \textbf{stop}
	\ENDIF
\ENDWHILE
\end{algorithmic}
}
\end{algorithm}


